Guessing the buffer bound for k-synchronizability

A communicating system is $k$-synchronizable if all of the message sequence charts representing the executions can be divided into slices of $k$ sends followed by $k$ receptions. It was previously shown that, for a fixed given $k$, one could decide whether a communicating system is $k$-synchronizable. This result is interesting because the reachability problem can be solved for $k$-synchronizable systems. However, the decision procedure assumes that the bound $k$ is fixed. In this paper we improve this result and show that it is possible to decide if such a bound $k$ exists.

==> SR.tex <==
% !TEX root = vmcai.tex







 %with unmatched sends}
In \cite{DBLP:conf/fossacs/GiustoLL20}, we have proven that knowing whether a system
is \kSable{k} for a given $k$ is decidable.
Here, we prove that finding whether there exists a $k$ such that the system is \kSable{k}  is decidable as well.

The intuition behind the algorithm is to build for each pair of global states all possible exchanges (i.e., sequences of sends followed by the corresponding receptions)  that satisfy causal delivery. Then we keep only those ones that cannot be divided into smaller ones, we call them prime exchanges. 
Finally if between each pair of global states only a finite number of exchanges is possible we determine their maximal lenght. This value, say $k$, is the only one admissible and  we test if all executions can be reorganized into $k$-exchanges by means of the algorithm in \cite{DBLP:conf/fossacs/GiustoLL20}. 
Let's see this construction more in detail.

\subsection{Causal delivelivery exchanges}

We start with the definition of exchange:
\begin{definition}[Exchange]
	An exchange $e=e_1 \cdot e_2 \cdots e_n $ is a sequence of actions such that:
	$\exists r \leq n$ such that $\forall i < r, e_i \in \sendSet$ and
	$\forall j \geq r, e_j \in \receiveSet$ and
	$\forall j$, if $e_j \in \receiveSet$ then $\exists i, e_i \in S$ and $ e_i
	\matches e_j$.
	
\end{definition}

Hence, for each   triple of states
$\triple$  and beginning with empty buffers, we check if we can build an \emph{exchange}: meaning that
$\globalstatelj$
can be reached only with sends from $\globalstateli$
and $\globalstatelf$
can be reached only with receptions from $\globalstatelj$. 
Languages $ \LangSauto$  and $\LangRauto$
correspond, respectively, to the sequences of messages that can be sent to go
from the state $\globalstateli$,
to $\globalstatelj$
and the sequences of receptions that can be done to go from $\globalstatelj$
to $\globalstatelf$
in the system (regardless of the actual state of buffers).
They are obtained as sort of projections from $P_{\system}$.

\begin{definition}[Automata $\AutSauto$ and $\AutRauto$]
	For  $P_{\system}$,
	finite state automaton $\AutSauto = (L_{\AutSauto}, \delta_{\AutSauto},
	\globalstate{l}^0_{\AutSauto},F)$ is defined as :
	\begin{itemize}
		\item $L_{\AutSauto} = L_{P_{\system}}$, $\globalstate{l}^0_{\AutSauto} =
		\globalstateli$ and  $F = \{ \globalstatelj \} $,
		\item $\delta_{\AutSauto} = \{ (\globalstate{l_m}, a,\globalstate{ l_{m'}})
		\mid (\globalstate{l_m}, a,\globalstate{ l_{m'}}) \in \delta_{P_{\system}}
		\wedge a \in \sendSet \}$
	\end{itemize}
	
	Automaton $\AutRauto = (L_{\AutRauto}, \delta_{\AutRauto},$ $
	\globalstate{l}^0_{\AutRauto},F)$ is defined as:
	\begin{itemize}
		\item $L_{\AutRauto} = L_{P_{\system}}$,  $\globalstate{l}^0_{\AutRauto} =
		\globalstatelj $ and $F = \{\globalstatelf \}$
		is a final state \item $\delta_{\AutRauto} = \{
		(\globalstate{l_m}, a, \globalstate{l_{m'}}) \mid (\globalstate{l_m},
		a,\globalstate{ l_{m'}}) \in \delta_{P_{\system}} \wedge a \in \receiveSet \}$
	\end{itemize}
	$\LangSauto$ and $\LangRauto$ denote respectively the regular languages of sends and receives.
\end{definition}


If any of these languages is empty, then the triple of states cannot correspond
to an exchange. Indeed, this means there is no path either between
$\globalstateli$ and $\globalstatelj$ with sends only, or between
$\globalstatelj$ and $\globalstatelf$ with receptions only.

% Note that $\LangSauto$ and $\LangRauto$ are regular languages.
% \begin{lemma}
% Languages $\LangSauto$ and $\LangRauto$ are regular.
% \end{lemma}
%
% \begin{proof}
% Let $\system$ be a system,  $P_{\system}$ be the product of automata of
% $\system$ and $\triple$ a triple of global states. We define $\AutSauto$ the
% automaton composed of selected states and transitions of $P_{\system}$, with
% $\globalstate{l_i}$ as initial state, $\globalstate{l_j}$ as final state, all
% send transitions from $P_{\system}$, and states concerned by these transitions.
% In the same way, $\AutRauto$ is the automaton composed with
% $\globalstate{l_j}$ as initial state, $\globalstate{l_f}$ as initial state, all
% receive transitions from $P_{\system}$ and states concerned by these
% transitions. Therefore, $\LangSauto$, and respectively, $\LangRauto$,
% corresponds to the language of automaton $\AutSauto$, resp. $\AutRauto$,
% and so there are regular languages.
% \end{proof}


VU LA CONSTRUCTION QUI SUIT SR PEUT ETRE CONSTRUIT JUSTE COMME PRODUIT DE L(SEND) ET L(REC)

Using $\AutSauto$ and $\AutRauto$, we can build an automaton that  selects only the sequences where all received messages have been effectively sent, and FIFO order and causal delivery are respected locally (we do not take into
account messages sent in other exchanges),  it is denoted
$\AutSRauto$.
%\item some of send messages may not be received (we do not verify at this point
%if causal delivery is satisfied),
% \item FIFO order is respected (\ie two matched messages sent to a same machine
% will be read in the same order as they were sent).
%
%
%
Intuitively, $\AutSRauto$ is a sort of ``synchronous" product automaton  between
$\AutSauto$ and $\AutRauto$.
Send actions that do not appear in
$\AutRauto$ are always considered.
These are unmatched sends that condemn the receiver buffer. Instead matched
sends are added if: (i) a send transition is possible from the state, (ii) its receive transition is also possible and (iii) the receiver buffer  is available.
%
More precisely, $\AutSRauto$  is a finite state automaton over the alphabet
$\Sigma = \{!,!?\} \times \paylodSet$. $! \Message{\amessage}{p}{q}$
represents unmatched send of message $\amessage$ sent from process $p$ to
process $q$ and $!? \Message{\amessage}{p}{q}$ is the  send with the matching
reception of message $\amessage$ from $p$ to $q$.

\begin{definition}[Automaton of matched and unmatched sends]
	For a system $\system$ and a triple of global states $\triple$, let
	$\AutSRauto = (L, \delta, \globalstate{l_0},F)$ be the automaton where:
	\begin{itemize}
		\item $L = \{ (\globalstate{l}_{m,n}, \condemned) \mid \globalstate{l}_m \in L_{\AutSauto}, \globalstate{l}_n \in
		L_{\AutRauto}, \condemned \subseteq \procSet \} $, each state is the combination of a
		state from the send automaton, a state from the receive automaton and  a set of
		processes representing the condemned buffers;
		\item $\globalstate{l_0} = (\globalstate{l}_{m,n}, \emptyset) \in L $
		where $\globalstate{l}_m = \globalstate{l}^0_{\AutSauto} $  and $\globalstate{l}_n = \globalstate{l}^0_{\AutRauto} $;
		\item $ F = \{ (\globalstate{l}_{m,n}, \condemned) \in L \mid \globalstate{l}_m \in F_{\AutSauto}, \globalstate{l}_n \in F_{\AutRauto}  , \condemned \subseteq \procSet \}$;
		\item for each $(\globalstate{l}_m,\send{p}{q}{\amessage},\globalstate{l}_{m'}) \in \delta_{\AutSauto}$:
		\begin{itemize}
			\item $((\globalstate{l}_{m,n}, \condemned), !\Message{\amessage}{p}{q}, (\globalstate{l}_{m',n}, \condemned \cup
			\{q\}) )\in \delta$ for all $\globalstate{l}_{n} \in L_{\AutRauto} $ and
			$\condemned \subseteq \procSet$;
			\item if $(\globalstate{l}_{n}, \rec{p}{q}{\amessage}, \globalstate{l}_{n'}) \in \delta_{\AutRauto}$  and $
			q \notin \condemned $ then $$ ((\globalstate{l}_{m,n}, \condemned), !?\Message{\amessage}{p}{q},
			(\globalstate{l}_{m',n'},\condemned)) \in \delta $$
		\end{itemize}
	\end{itemize}
\end{definition}

This is an example of the construction.
\begin{example}\label{example:aut_SR}
	Let $\system$ be a system composed of automata $p,q$ and $r$.
	For the triple $\triple$ where $\globalstateli = (0,0,0), \globalstatelj =
	(2,0,1)$ and $\globalstatelf = (2,1,2)$,  automata $\AutSauto$ and
	$\AutRauto$ are depicted in
	Fig~\ref{figure:ex_aut_SR} followed by the resulting automaton
	$\AutSRauto$. As we can see, $$\LangSRauto =
	((\Action{!?}{\Message{a}{p}{r}}
	\Action{!?}{\Message{b}{r}{q}}) + (  \Action{!?}{\Message{b}{r}{q}}
	\Action{!?}{\Message{a}{p}{r}} ))\Action{!}{ \Message{c}{p}{q}}.$$
	
	\begin{figure}[t]
		\input{exmp_aut_SR}
		\caption{Example of generation of automaton $\protect\AutSRauto$ with $\protect\globalstateli = (0,0,0)$, $\protect\globalstatelj = (2,0,1)$, and $\protect\globalstatelf = (2,1,2)$}
		\label{figure:ex_aut_SR}
	\end{figure}
	
\end{example}



%\input{proof_lemma_SR_causal}

%\input{proof_lemma_Aut_SR}

\begin{remark}
	The construction of $\AutSRauto$ works only for mailbox communication. It
	would not be correct for peer-to-peer communication, where a buffer would be
	condemned only for the precise sender  and not for all processes.
\end{remark}

The last step is to verify that causal delivery is satisfied with respect to other triples.

IF L->L' IN SR THEN BUILD L,B--> L,B' AS FOLLOWS

 The first one is to ensure, while reading $w$, that the extended conflict
graph remains acyclic. The only way to create a cycle is to use an $\cgedgeD{SS}$ edge generated by Rule 4, since
these are the only edges that ``go back in time''. So, for every $!?\amessage^{p\to q}$, one should be sure
that $p\not\in C_{S,q}$. The second task is to ensure that $\Br^{(0)}\Tr{msc(w)}\Br^{(1)}$ for some fixed
functions $\Br^{(0)}$ and $\Br^{(1)}$. For this, the automaton updates $\Br$ while reading every symbol of $w$,
starting with $\Br=\Br^{(0)}$. We define
the two relations $\Br \tr{!?\amessage^{p\to q}}\Br'$ and 
$\Br \tr{!\amessage^{p\to q}}\Br'$. In the remainder, we let $\Br(p)=(C_{S,p},C_{R,p})$,
$\Br'(p)=(C_{S,p}',C_{R,p}')$ and $\Br^{(0)}(p)=(C_{S,p}^{(0)},C_{R,p}^{(0)})$ for all $p$.
\begin{itemize}
	\item $\Br \tr{!?\amessage^{p\to q}}\Br'$ holds if (1) $p\not\in C_{S,q}$ and (2) for all $r\in\procSet$, the following holds: let the intermediate set $C_{S,r}''$ be defined by
	$$
	C_{S,r}''=\left\{\begin{array}{l}
		C_{S,r}\cup\{p\} \mbox{ if }p\in C_{R,r}^{(0)}\mbox{ or }q\in C_{R,r}\\
		C_{S,r}\mbox{ otherwise}
	\end{array}\right.
	$$
	Then 
	$$
	C_{S,r}'=\left\{\begin{array}{l}
		C_{S,r}''\cup C_{S,q} \mbox{ if }p\in C_{S,r}''\\
		C_{S,r}\mbox{ otherwise}
	\end{array}\right.
	\qquad\mbox{and}\qquad
	C_{R,r}'=\left\{\begin{array}{l}
		C_{R,r}\cup C_{R,q} \mbox{ if }p\in C_{S,r}''\\
		C_{R,r}\mbox{ otherwise}
	\end{array}\right.
	$$
	\item $\Br \tr{!\amessage^{p\to q}}\Br'$ holds if for all $r\in\procSet$, 
	$$
	C_{S,r}'=\left\{\begin{array}{l}
		C_{S,r}\cup \{p\} \mbox{ if }q=r\mbox{ or } q\in C_{R,r}\\
		C_{S,r}\mbox{ otherwise}
	\end{array}\right.
	\qquad\mbox{and}\qquad
	C_{R,r}'=C_{R,r}
	$$
	
\end{itemize}

\subsection{Prime exchanges}

AS ETIENNE

\subsection{Computing the size}

For each triple of states $\triple$ there exist a finite state automaton $\SR(\globalstateli,\Br_i,\globalstatelf,\Br_f) )$. Next we define the set of reachable causal delivery and prime  triples. 

\begin{definition}[Reachable triples]
	
Let $\mathcal{S}$ be the least set of regular languages  $\LSR{\globalstateli,\Br_i,\globalstatelf,\Br_f}$ that verifies
the following three conditions:
\begin{enumerate}
	\item $\LSR{\globalstateli,\Br_i,\globalstatelf,\Br_f}$ is not empty and prime
	\item for any $(\globalstatelf,\Br_f)$, the
	language $\LSR{\globalstate{l_0},\Br_0,\globalstatelf,\Br_f}$ is in $\mathcal S$
	\item for any $\globalstate{l_1},\globalstate{l_2},\globalstate{l_3}$ and any $\Br_1,\Br_2,\Br_3$, if
	$\LSR{\globalstate{l_1},\Br_1,\globalstate{l_2},\Br_2}\in \mathcal S$  then $\LSR{\globalstate{l_2},\Br_2,\globalstate{l_3},\Br_3}\in \mathcal S$.
\end{enumerate}

Let $w_{\globalstateli,\Br_i,\globalstatelf,\Br_f}$ be the regular expression representing language $\LSR{\globalstateli,\Br_i,\globalstatelf,\Br_f}$
\end{definition}

The last thing that remains it is to compute the size of the biggest exchange, that is the size of its regular expression.
$$
\begin{array}{lll}
|w| ::= & 1 & \text{if } w = !?\amessage^{p\to q} \text{ or } w = !\amessage^{p\to q}  \\  
& |w_1| + |w_2| & \text{if } w = w_1 \cdot w_2 \\
& max(|w_1|, |w_2|) \quad & \text{if } w = w_1 + w_2 \\
& \infty & \text{if } w = w_1^* 

\end{array}
$$

Notice that if the regular expression contains a kleene star operator it means, since the exchange is prime, that its size can grow unboundedly.  

Let $k = max\{|w_{\globalstateli,\Br_i,\globalstatelf,\Br_f}| \mid \LSR{\globalstateli,\Br_i,\globalstatelf,\Br_f} \in \mathcal{S} \} $.
If $k \neq \infty$ the only thing that remains to do is to use the algorithm in \cite{DBLP:conf/fossacs/GiustoLL20} to verify that all executions have been captured. If the procedures answers positevely that the system is k-synchronizable.



==> core.tex <==
% !TEX root = vmcai.tex


 %with unmatched sends}
In \cite{DBLP:conf/fossacs/GiustoLL20}, we have proven that knowing whether a system
is \kSable{k} for a given $k$ is decidable.
Here, we prove that finding whether there exists a $k$ such that the system is \kSable{k}  is decidable as well.

The intuition behind the algorithm is to build all possible exchanges of a system (i.e., sequences of sends followed by the corresponding receptions), pick the
size of the largest one and, if it exists, test if it represents a good candidate.
 Thus, we consider each triple of states
$\triple$  and beginning with empty buffers, we check if we can build an \emph{exchange}: meaning that
$\globalstatelj$
can be reached only with sends from $\globalstateli$
and $\globalstatelf$
can be reached only with receptions from $\globalstatelj$.

\begin{definition}[Exchange]
An exchange $e=e_1 \cdot e_2 \cdots e_n $ is a sequence of actions such that:
$\exists r \leq n$ such that $\forall i < r, e_i \in \sendSet$ and
$\forall j \geq r, e_j \in \receiveSet$ and
 $\forall j$, if $e_j \in \receiveSet$ then $\exists i, e_i \in S$ and $ e_i
 \matches e_j$.

\end{definition}

To increase readability we list here the steps that are necessary  to decide whether there exists a $k$ such that the system is \kSable{k} :
\begin{enumerate}[Step 1.]
  \item We first build the languages representing the send and
  receive capabilities of each triple $\triple$.
  \item Then we compose these two languages to consider only suitable sequences of sends and receives (e.g.,  sequences that satisfy causal delivery).
  \item Next, we build a FSA that collect the causal relationships among all the triples.
  \item We consider all reachable triples in the FSA and we compute their sizes. Let $k$ be the maximal one (if it
  exists).
  \item Finally, we use the algorithm in \cite{DBLP:conf/fossacs/GiustoLL20} to
  check whether the system is \kSable{k}. If the algorithm answers positively, then the
  system is \kSable{k}, other\-wise there is no $k$ such that the system is
  \kSable{k}.
\end{enumerate}

\subsection*{Step 1. Send and receive languages}

Languages $ \LangSauto$  and $\LangRauto$
correspond, respectively, to the sequences of messages that can be sent to go
from the state $\globalstateli$,
to $\globalstatelj$
and the sequences of receptions that can be done to go from $\globalstatelj$
to $\globalstatelf$
in the system (regardless of the actual state of buffers).
They are obtained as sort of projections from $P_{\system}$.

\begin{definition}[Automata $\AutSauto$ and $\AutRauto$]
For  $P_{\system}$,
finite state automaton $\AutSauto = (L_{\AutSauto}, \delta_{\AutSauto},
\globalstate{l}^0_{\AutSauto},F)$ is defined as :
\begin{itemize}
\item $L_{\AutSauto} = L_{P_{\system}}$, $\globalstate{l}^0_{\AutSauto} =
\globalstateli$ and  $F = \{ \globalstatelj \} $,
\item $\delta_{\AutSauto} = \{ (\globalstate{l_m}, a,\globalstate{ l_{m'}})
\mid (\globalstate{l_m}, a,\globalstate{ l_{m'}}) \in \delta_{P_{\system}}
\wedge a \in \sendSet \}$
\end{itemize}

Automaton $\AutRauto = (L_{\AutRauto}, \delta_{\AutRauto},$ $
\globalstate{l}^0_{\AutRauto},F)$ is defined as:
\begin{itemize}
\item $L_{\AutRauto} = L_{P_{\system}}$,  $\globalstate{l}^0_{\AutRauto} =
\globalstatelj $ and $F = \{\globalstatelf \}$
is a final state \item $\delta_{\AutRauto} = \{
(\globalstate{l_m}, a, \globalstate{l_{m'}}) \mid (\globalstate{l_m},
a,\globalstate{ l_{m'}}) \in \delta_{P_{\system}} \wedge a \in \receiveSet \}$
\end{itemize}
$\LangSauto$ and $\LangRauto$ denote respectively the regular languages of sends and receives.
\end{definition}


If any of these languages is empty, then the triple of states cannot correspond
to an exchange. Indeed, this means there is no path either between
$\globalstateli$ and $\globalstatelj$ with sends only, or between
$\globalstatelj$ and $\globalstatelf$ with receptions only.

% Note that $\LangSauto$ and $\LangRauto$ are regular languages.
% \begin{lemma}
% Languages $\LangSauto$ and $\LangRauto$ are regular.
% \end{lemma}
%
% \begin{proof}
% Let $\system$ be a system,  $P_{\system}$ be the product of automata of
% $\system$ and $\triple$ a triple of global states. We define $\AutSauto$ the
% automaton composed of selected states and transitions of $P_{\system}$, with
% $\globalstate{l_i}$ as initial state, $\globalstate{l_j}$ as final state, all
% send transitions from $P_{\system}$, and states concerned by these transitions.
% In the same way, $\AutRauto$ is the automaton composed with
% $\globalstate{l_j}$ as initial state, $\globalstate{l_f}$ as initial state, all
% receive transitions from $P_{\system}$ and states concerned by these
% transitions. Therefore, $\LangSauto$, and respectively, $\LangRauto$,
% corresponds to the language of automaton $\AutSauto$, resp. $\AutRauto$,
% and so there are regular languages.
% \end{proof}


\subsection*{Step 2. Suitable sequences}
Using $\AutSauto$ and $\AutRauto$, we can build an automaton that  selects only the sequences where all received messages have been effectively sent, and FIFO order and causal delivery are respected locally (we do not take into
account messages sent in other exchanges),  it is denoted
$\AutSRauto$.
%\item some of send messages may not be received (we do not verify at this point
%if causal delivery is satisfied),
% \item FIFO order is respected (\ie two matched messages sent to a same machine
% will be read in the same order as they were sent).
%
%
%
 Intuitively, $\AutSRauto$ is a sort of ``synchronous" product automaton  between
 $\AutSauto$ and $\AutRauto$.
 Send actions that do not appear in
 $\AutRauto$ are always considered.
These are unmatched sends that condemn the receiver buffer. Instead matched
sends are added if: (i) a send transition is possible from the state, (ii) its receive transition is also possible and (iii) the receiver buffer  is available.
%
 More precisely, $\AutSRauto$  is a finite state automaton over the alphabet
 $\Sigma = \{!,!?\} \times \paylodSet$. $! \Message{\amessage}{p}{q}$
 represents unmatched send of message $\amessage$ sent from process $p$ to
 process $q$ and $!? \Message{\amessage}{p}{q}$ is the  send with the matching
 reception of message $\amessage$ from $p$ to $q$.

 \begin{definition}[Automaton of matched and unmatched sends]
For a system $\system$ and a triple of global states $\triple$, let
$\AutSRauto = (L, \delta, \globalstate{l_0},F)$ be the automaton where:
\begin{itemize}
\item $L = \{ (\globalstate{l}_{m,n}, \condemned) \mid \globalstate{l}_m \in L_{\AutSauto}, \globalstate{l}_n \in
L_{\AutRauto}, \condemned \subseteq \procSet \} $, each state is the combination of a
state from the send automaton, a state from the receive automaton and  a set of
processes representing the condemned buffers;
\item $\globalstate{l_0} = (\globalstate{l}_{m,n}, \emptyset) \in L $
where $\globalstate{l}_m = \globalstate{l}^0_{\AutSauto} $  and $\globalstate{l}_n = \globalstate{l}^0_{\AutRauto} $;
\item $ F = \{ (\globalstate{l}_{m,n}, \condemned) \in L \mid \globalstate{l}_m \in F_{\AutSauto}, \globalstate{l}_n \in F_{\AutRauto}  , \condemned \subseteq \procSet \}$;
\item for each $(\globalstate{l}_m,\send{p}{q}{\amessage},\globalstate{l}_{m'}) \in \delta_{\AutSauto}$:
\begin{itemize}
\item $((\globalstate{l}_{m,n}, \condemned), !\Message{\amessage}{p}{q}, (\globalstate{l}_{m',n}, \condemned \cup
\{q\}) )\in \delta$ for all $\globalstate{l}_{n} \in L_{\AutRauto} $ and
$\condemned \subseteq \procSet$;
\item if $(\globalstate{l}_{n}, \rec{p}{q}{\amessage}, \globalstate{l}_{n'}) \in \delta_{\AutRauto}$  and $
q \notin \condemned $ then $$ ((\globalstate{l}_{m,n}, \condemned), !?\Message{\amessage}{p}{q},
(\globalstate{l}_{m',n'},\condemned)) \in \delta $$
\end{itemize}
\end{itemize}
\end{definition}

This is an example of the construction.
\begin{example}\label{example:aut_SR}
  Let $\system$ be a system composed of automata $p,q$ and $r$.
  For the triple $\triple$ where $\globalstateli = (0,0,0), \globalstatelj =
  (2,0,1)$ and $\globalstatelf = (2,1,2)$,  automata $\AutSauto$ and
  $\AutRauto$ are depicted in
  Fig~\ref{figure:ex_aut_SR} followed by the resulting automaton
  $\AutSRauto$. As we can see, $$\LangSRauto =
  ((\Action{!?}{\Message{a}{p}{r}}
  \Action{!?}{\Message{b}{r}{q}}) + (  \Action{!?}{\Message{b}{r}{q}}
  \Action{!?}{\Message{a}{p}{r}} ))\Action{!}{ \Message{c}{p}{q}}.$$

  \begin{figure}[t]
    \input{exmp_aut_SR}
    \caption{Example of generation of automaton $\protect\AutSRauto$ with $\protect\globalstateli = (0,0,0)$, $\protect\globalstatelj = (2,0,1)$, and $\protect\globalstatelf = (2,1,2)$}
    \label{figure:ex_aut_SR}
  \end{figure}

\end{example}

To show that all the sequences in $\LangSRauto$ satisfy causal delivery we introduce a function  $\func{w}{\varepsilon}$ that allows to transform
words $w \in \LangSRauto$ into sequences of actions run by the system.
The resulting sequence of actions is build by first taking all sends and then adding all the
matched receptions in the same order of the sends.

\begin{definition}
For a sequence of messages $m \in \Sigma^*$,
we define $\func{m}{\varepsilon}$ as:
$$
\func{m}{w} =  \left\{
	\begin{array}{l l}
		w & \mbox{ if } m = \varepsilon  \\
		!a  \cdot \func{m'}{w} & \mbox{ if } m = !a  \cdot r' \\
		!a \cdot \func{m'}{w \cdot ?a} & \mbox{ if } m = !?a \cdot r' \\
	\end{array}
\right.
$$
% For $\func{m}{\varepsilon} =  s_1 \cdots s_n \cdot r_1 \cdots r_{n'}$, $s_i \in
% S^*$ and $r_i \in R^*$, we denote  $\func{m}{\varepsilon}_S = s_1 \cdots s_n$
% and $\func{m}{\varepsilon}_R = r_1 \cdots r_{n'}$.
%\todo{utile ?}
\end{definition}
{\color{red} commentaire post-soumission : typo confusion entre m' et r'}



\begin{lemma}\label{lemma:SR_causal}
  For a system $\system$ and a triple $\triple$, if $w \in \LangSRauto$ then
  $MSC(\func{w}{\varepsilon})$ satisfies causal delivery.
\end{lemma}

%\input{proof_lemma_SR_causal}


Each of the sequences in $\LangSRauto$ belongs to $\LangSauto$ and, if
restricted to matched messages, they belong to $\LangRauto$.
If $\LangSRauto = \emptyset$, the concerned triple is ignored
since there is no corresponding sequence of actions in the global system.

Next lemma shows that for each exchange in $\triple$ there exists a word in
$\LangSRauto$ that corresponds to it.
\begin{lemma}\label{lemma:Aut_SR}
For $e = s_1 \cdots s_n \cdot r_1 \cdots r_{n'}$ with $s_1 \cdots s_n \in S^*$
and  $r_1 \cdots r_{n'} \in R^*$, if there is a triple $\triple$ and $ \B, \B'$
such that $$(\globalstateli, \B_{\emptyset}) \xRightarrow{s_1 \cdots s_n}
(\globalstatelj, \B) \xRightarrow{r_1 \cdots r_{n'}} (\globalstatelf,
\B')$$ then there is $w \in \Language{\AutSRauto}$ such that $msc(e) =
msc(\func{w}{\varepsilon})$.
\end{lemma}

%\input{proof_lemma_Aut_SR}

\begin{remark}
  The construction of $\AutSRauto$ works only for mailbox communication. It
  would not be correct for peer-to-peer communication, where a buffer would be
  condemned only for the precise sender  and not for all processes.
\end{remark}

\subsection*{Step 3. Causal exchanges}
MSCs representing words of $\AutSRauto$ verify causal delivery only locally.
However, if $\globalstateli$ is not the initial state of the system, there
have been other messages that have been sent before. So we need to verify causal delivery
ta\-king into account the past (intuitively what buffers are condemned because of
previous unmatched sends).
As shown in following Example~\ref{ex:why_decomp}, the language of $\AutSRauto$ may
contain both words that verify causal delivery and words that do not.
% Within language $\AutSRauto$, maybe some
% words verify causal delivery and some do not, because they do not contain the
% same action, as we can see in Example~\ref{ex:why_decomp}.

\begin{example} \label{ex:why_decomp}
For a system $\system$ composed of automata $p$ and $q$, as depicted in
Fig.~\ref{fig:ex_why_decomp}(a), and the triple $\triple$ where $\globalstateli =
(1,0), \globalstatelj = (3,0)$ and $\globalstatelf = (3,0)$, the resulting
automaton $\AutSRauto$ is given in Fig.~\ref{fig:ex_why_decomp}(b).
As we can see, $\LangSRauto = (\Action{!}{\Message{b}{p}{q}} +
\Action{!?}{\Message{b}{p}{q}}) \Action{!}{\Message{c}{p}{q}}$. Nonetheless, if
we take into consideration message $a$ that has been sent in the past to reach global
state $\globalstateli$, the MSC of the sequence of action
$\Action{!}{\Message{a}{p}{q}}\Action{!}{\Message{b}{p}{q}}\Action{!}{\Message{c}{p}{q}}$
verifies causal delivery but the one of
$\Action{!}{\Message{a}{p}{q}}\Action{!?}{\Message{b}{p}{q}}\Action{!}{\Message{c}{p}{q}}$
does not,
since $a$ is sent before $b$ by the same sender and $b$ can not be received as
$a$ is unmatched.
{\color{red} Figure changée depuis version soumise}
\end{example}



\begin{figure}[t]
\begin{center}
\input{exmp_why_decomp}
\caption{\textbf{(a)} depicts system $\system$ and \textbf{(b)} automaton $\protect\AutSRauto$ for $\protect\globalstateli = (1,0), \protect\globalstatelj = (3,0), \protect\globalstatelf =(3,0)$}
\label{fig:ex_why_decomp}
\end{center}
\end{figure}


Therefore,
we need a mechanism to consider past causal relationships.
We know that, as shown in Theorem 2 of \cite{DBLP:conf/fossacs/GiustoLL20},
 causal delivery can be
verified by checking that there exists no cycle $v \cgedgeD{SS} v$ in the
extended conflict graph of a given MSC.



The idea is to extend Theorem 2 in \cite{DBLP:conf/fossacs/GiustoLL20} to handle
conflict graphs built from the regular expression representing the words in
$\LangSRauto$. We will see that past causal relationship can be handled in the
same way as in \cite{DBLP:conf/fossacs/GiustoLL20}. We keep a pair of sets $\Br
= (\Crxp{S}{p}, \Crxp{R}{p})$ that for each process stores the causal
relationships related to the sender or respectively the receiver. The only thing
that remains is to show how to build a conflict graph from a regular expression.
We have observed that there could be words in the same language that satisfy
causal delivery and others that do not. The idea is that we can consider
families of sequential behaviours, \ie sublanguages of $\AutSRauto$ that can be
characterized by a regular expression that does not contain choice operators.
%
% A single conflict graph for all behaviours of $\AutSRauto$ would not be enough.
% It is clear that all behaviours (words) in $\LangSRauto$ cannot be
% represented by a single MSC. Indeed we can only represent families of sequential
% behaviours, \ie sublanguages of $\AutSRauto$ that can be characterized by a
% regular expression that do not contain choice operators.
%
Intuitively, this
corresponds to a path (with possibly some cycles) from the initial state to the
final state in  $\AutSRauto$.
Recall that
for each regular expression there exists an equivalent expression that only
contains choice operators at top level (\cite{cousot2019calculational}), this is
called Disjunctive Normal Form.
 Each disjunction of this form designates a path in $\AutSRauto$ described
 by a sequence of sends matched or unmatched in an fixed order belonging to
 $\LangSRauto$.
 On top of this, we have observed that the number of unfoldings of a star operator plays a role in determining whether a sequence of actions satisfies causal delivery or not. Hence
 we consider a variant of the definition of DNF where we
 explicitly take zero or more occurrences of the expressions under the star
 operators.

\begin{definition}[Decomposition of $\LangSRauto$]
For $r$  regular expression, the decomposition $\decomp{r}$ is:
\begin{itemize}
\item if $r= \varepsilon$ then $\decomp{r} = \varepsilon$ ;
\item if $r = v \in \{!?,!\} \times \paylodSet$ then $ \decomp{r} = \{v\}$.
{\color{red} commentaire post-soumission : il manque p et q en exposant}
\item if $r=r_1 + r_2$ then $\decomp{r_1 + r_2} = \decomp{r_1} \cup \decomp{r_2}$
\item  if $r=r_1^*$ then $\decomp{r_1^*} =
\{ (\bullet_{r_1^i \in I} (r_1^i)^*)^* \mid I \in 2^{\decomp{r_1}}\}$
%\bigcup_{I \in 2^{ \decomp{r_1}} } \{(\bullet_{r_1^i \in I}
%(r_1^i)^* )^*\}$
\item  if $r=r_1 r_2$ then $\decomp{r_1r_2} = \{ r_1^i r_2^j \mid r_1^i \in \decomp{r_1} $ and $r_2^j
\in \decomp{r_2}\}$
\end{itemize}
The decomposition $\decomp{\LangSRauto}$ is denoted $\decompsetauto$.
\end{definition}

The following are two examples of decompositions:
\begin{example}
\begin{align*}
  \decomp{ (\Action{!}{\Message{a}{p}{q}}+\varepsilon )\Action{!?}{\Message{b}{q}{p} } ) } =
  \{& \Action{!}{\Message{a}{p}{q}}\Action{!?}{\Message{b}{q}{p} }, \Action{!?}{\Message{b}{q}{p} } \} \\
  \decomp{\Action{!?}{\Message{a}{p}{q}} (\Action{!?}{\Message{b}{p}{q}} + \Action{!?}{\Message{c}{p}{q}} )^* \Action{!}{\Message{d}{q}{p}} ) }=
  \{
  &\Action{!?}{\Message{a}{p}{q}} \Action{!}{\Message{d}{q}{p}}, \\
  & \Action{!?}{\Message{a}{p}{q}} (\Action{!?}{\Message{b}{p}{q}})^* \Action{!}{\Message{d}{q}{p}}, \\
  &\Action{!?}{\Message{a}{p}{q}} (\Action{!?}{\Message{c}{p}{q}})^* \Action{!}{\Message{d}{q}{p}}, \\
  &\Action{!?}{\Message{a}{p}{q}} ((\Action{!?}{\Message{b}{p}{q}})^*(\Action{!?}{\Message{c}{p}{q}})^*)^* \Action{!}{\Message{d}{q}{p}}
  \}
\end{align*}
\end{example}

Next lemma shows that our variant is correct and that the languages are preserved. By abuse of notation when writing $r \equiv \decomp{r}$ we mean that the language of regular expression $r$ is equivalent to the language of its decomposition.
\begin{lemma}\label{lemma:SR_D}
 $r \equiv \decomp{r}$.
\end{lemma}

%\input{proof_lemma_SR_D}

Next, we  build the conflict graph, that will be completed with the
information about the past to obtain the extended conflict graph.

First, we modify each regular expression replacing star operators with a new
operator $\dotstar$ that explicits their first and last iteration. Moreover,
each occurence of a symbol is set apart by a fresh pedex: e.g.
$\transf{(\Action{!?}{\Message{\amessage}{p}{q}})^*} =
\Action{!?}{\Message{\amessage_0}{p}{q}} \dotstar
\Action{!?}{\Message{\amessage_1}{p}{q}}$.
This is called the transformed regular expression. In the following definition
$\dagger \in \{!?, !\}$ and $\amessage \in \paylodSet$.

\begin{definition}[Transformed regular expression]
  The transformed regular expression $\transf{exp}$ of a regular expression
  $exp$ without choice operators is:
  $$\transf{exp}= emb(dup(exp))$$
  where function $dup$ replaces star operators:
  $$ dup(exp) = \left\{
  	\begin{array}{l l}
      exp & \mbox{ if } exp = \varepsilon \mbox{ or } exp = \dagger \amessage \\
      dup(e_1)\cdot dup(e_2) & \mbox{ if } exp = e_1\cdot e_2 \\
      dup(e_1)\dotstar dup(e_1) & \mbox{ if } exp = e_1^* \\
  	\end{array}
  \right.
  $$
  and function $emb$ adds fresh pedexes to distinguish between occurences of the same $\amessage$.
  % :
  % $$emb(exp,g) = \left\{
  % \begin{array}{l l}
  %   \varepsilon & \mbox{ if } exp = \varepsilon \\
  %   \dagger \amessage_{g(\amessage)} \cdot
  %       emb(exp', g[g(\amessage) \leftarrow g(\amessage)+1]) & \mbox{ if } exp = \dagger \amessage \cdot exp' \\
  % \end{array}
  % \right.
  % $$
  % for $g: V \rightarrow \mathbb{N}$, where $\forall \amessage \in \paylodSet$, $g(\amessage)= 0$ at the initialization.
\end{definition}

Then we project the transformed regular expression on each machine to detect which dependency exists between two consecutive actions on the
same machine. Two consecutive sends on the same machine have an edge $SS$
between them, a send followed by a reception have an edge $SR$ and two receptions
have an edge $RR$. Each projection is encoded into a part of conflict graph,
with sets $V$ of vertices and $E$ of edges. In the rest of the encoding, sets $I$ and $F$ are used to recognize respectively the first and the last symbol of an expression.


%
%
% \begin{definition}[Transformation of a regular expression]
%   Let $r$ be a regular expression. The transformed regular expression $\transf{r}$
%   is defined as followed:
%   \begin{itemize}
%     \item[\textnormal{BASE}] for $r = \dagger v$,$ \dagger v \in \Sigma$,
%     $\transf{r} = \dagger v_0$;
%     \item[\textnormal{REC}] $r_1, r_2 \in r $:
%     \begin{itemize}
%       \item $\transf{r_1 \cdot r_2} = r_1 \cdot r_2$;
%       \item  $\\transf{r_1^*} = (r_1) \dotstar  (dup(r_1))$
%     \end{itemize}
%     where for $v\in \paylodSet, \dagger \in \{!,!?\} $,
%     \begin{itemize}
%       \item $dup( \dagger v_i \cdot r_1') = \dagger v_{i + g(\dagger v)} \cdot
%       dup(r_1')$ and
%       \item $g(\dagger v) = k $ such that $v_{k-1} \in r_1 $ and $v_{k} \notin r_1$.
%     \end{itemize}
%
%   \end{itemize}
% \end{definition}


\begin{definition}[Projection of a transformed regular expression]
Let $exp$ be a transformed regular expression. The projection $exp \proj{pX}$
for $p \in \procSet$ and $X \in \{ S,R \}$, with $q \in \procSet$, $\amessage \in \paylodSet$ is:
$$
exp \proj{pX} = \left\{
\begin{array}{l l}
  \Message{v}{p}{q} & \mbox{ if } (exp = \Action{\dagger}{\Message{\amessage}{p}{q}} \mbox{ and } X = S) \\
  &  \quad  \mbox{ or } (exp = \Action{!?}{\Message{\amessage}{p}{q}} \mbox{ and } X = R) \\
  e_1 \proj{pX} \cdot e_2 \proj{pX} & \mbox{ if } exp = e_1 \cdot e_2 \\
  e_1 \proj{pX} \dotstar~ e_2 \proj{pX} &\mbox{ if } exp = e_1 \dotstar e_2 \mbox{ and } e_1 \proj{pX} \neq \varepsilon  \\
  \varepsilon & \mbox{ otherwise } \\
\end{array}
\right.
$$

\end{definition}

The conflict graph of a transformed regular expression is composed of edges SS
built by projection on sends of each machine, edges RR built by projection on
receptions of each machine, and edges SR linking ends of sends to beginnings of
receptions. The star edges ($\cgedgeS$) link the first iteration at the
last one of a star operator.


\begin{definition}[Encoding of a regular expression]
For a projection of a transformed regular expression $e = \transf{exp}
\proj{pX}$ with $X \in \{S,R\}$,
let $ \encode{e} = (V,E,I,F)$ be its encoding,
where $\encode{e}_V$ is a set of
vertices, $\encode{e}_E$ a set of edges, $\encode{e}_I$ a set of starting
points and $\encode{e}_F$ a set of ending
points, defined as below:

\begin{itemize}
\item for $e = \amessage_i$,  $\encode{e} = (\{ \amessage_i
\}, \emptyset, \{ \amessage_i \}, \{ \amessage_i \} )$;
\item for $e_1,e_2 \in e$:
\begin{align*}
 \encode{ e_1 \cdot e_2 } = (
 			& \encode{e_1}_V \cup \encode{e_2}_V, \\
 			& \encode{e_1}_E \cup \encode{e_2}_E \cup \{a \cgedge{XX} b \mid a \in
 			\encode{e_1}_F, b \in\encode{e_2}_I\},\\
  		& \encode{e_1 }_I, \encode{e_2}_F ) \\
\encode{ (e_1 \dotstar e_2) } = (
      & \encode{e_1}_V \cup \encode{e_2}_{V} , \\
			&	 \encode{e_1}_E \cup \encode{e_2}_{E} \cup  \{ a \cgedgeS b \mid a
      \in \encode{e_1}_F, b \in \encode{e_2}_{I} \}, \\
    	&\encode{e_1}_I, \encode{e_2}_{F})
\end{align*}
\end{itemize}

\end{definition}


Finally, we can add SR edges using both projections on send and receive actions.
Notice that, by construction of $\AutSRauto$, we know that there can not be RS edges.

\begin{definition}[Conflict graph of a regular expression]
Let $exp$ be a regular expression.
The associated conflict graph is $\scgraph{exp} =
(V,E)$ where:
\begin{align*}
V = &  \bigcup _{p\in\procSet}   \encode{\transf{exp}\proj{pS}}_V  \\
E = &  \bigcup_{p\in\procSet}
    \big( \encode{\transf{exp} \proj{pS} }_E \cup
        \encode{\transf{exp} \proj{pR}}_E \\
      & \qquad \cup \{ a \cgedge{SR} b \mid
		        a \in \encode{ \transf{exp} \proj{pS} }_F,
            b \in \encode{\transf{exp} \proj{pR} }_I \}\big) \\
\end{align*}
\end{definition}




\begin{example}[Building a conflict graph from a regular expression]\label{ex:cgfromregexp}
\input{exmp_build_conflict_graph.tex}
\end{example}

Lastly, we give the definition of extended conflict graph that takes into
account the information on past causal relationships. The definition is an
immediate generalisation of extended edges defined in Section 4 in
\cite{DBLP:conf/fossacs/GiustoLL20} and recalled in Section \ref{sec:prelim}.


\begin{definition}[Extended conflict graph of a regular expression]
Let $exp$ be a regular expression such that $\scgraph{exp} = (V,E)$.
% and $\globalstate{l_i}$ a reachable state for some $B$.
We define  $\ecgraph{exp,\Br} = (V',E')$ the associated extended conflict graph for some $\Br$ such that
$V' = V \cup \{\lambdanode_p \mid p \in \procSet \}$ and
\begin{align}
E' = \ &  E \cup E'' \nonumber \\
 \cup \ &
   \{\lambdanode_p \cgedge{SX} v \mid\procofactionv{X}{v} \in C_{S,p}
   \with   v\cap X\neq\emptyset \mbox{ for some }X\in\{S,R\}\}   \label{eq:SS}
  \\ \cup \  &
 \{\lambdanode_p \cgedge{SS} v\mid \procofactionv{X}{v} \in C_{R,p}
 \with v \cap R \neq \emptyset \mbox{ for some }X\in\{S,R\}\}  \label{eq:RR}
  \\ \cup \ &
\{ \lambdanode_p \cgedge{SS} v \mid  \procofactionv{R}{v} \in C_{R,p}  \with  v
\mbox{ is unmatched} \}   \label{eq:unmatchedSS}
  \\ \cup \ &
 \{ v \cgedge{SS} \lambdanode_p \mid \procofactionv{R}{v} = p \with   v \cap R
 \neq \emptyset \} %\label{eq:vSS}
\ \cup \
\{ \lambdanode_q \cgedge{SS} \lambdanode_p \mid p \in C_{R,q}  \}\label{eq:psiSS}
\end{align}
where $E''$  is the set of extended edges built by Rules in
Fig.~\ref{fig:conflict-graph-extension} and Rule 6 below.
 \end{definition}
\begin{center}
\AxiomC{$ v_1 \cgedgeS v_2$}
\LeftLabel{(Rule 6)}
\UnaryInfC{$v_1 \cgedgeD{SS} v_2$}
\DisplayProof
\end{center}


\begin{figure}[t]
\begin{prooftree}
\AxiomC{\small \stackanchor{
$r \in \decompsetauto$ }
		{\stackanchor	{}
			{ \stackanchor	{$\mbox{ for all }p\in\procSet\quad
      \Br(p)=(\Crxp{S}{p},\Crxp{R}{p}) \mbox{ and }
      \Br'(p)=(\Crxp{S}{p}',\Crxp{R}{p}'), $}
				{\stackanchor { $\mathsf{Unm}_p=\{\lambdanode_p\}\cup\{v\mid v  \mbox {
        is unmatched,  } \receiver{v}=p\}$}
					{\stackanchor { $\Crxp{X}{p}'= \Crxp{X}{p}
					 \cup  \{p \mid p  \in  \Crxp{X}{q}, v \cgedgeD{SS} \lambdanode_q,
           (\receiver{v} = p \mbox{ or } v = \lambdanode_p)\} ~\cup$}
		{\stackanchor 	{
		\stackanchor{$ \{\procofaction{X}{v} \mid v \in\mathsf{Unm}_p\cap V, X = S
		\}\cup  \{\procofactionv{X}{v'} \mid v\cgedgeD{SS} v', v\in\mathsf{Unm}_p, v
		\cap X \neq \emptyset\}
		$}}
 		{$\mbox{for all } p \in \procSet, p\not\in \Crxp{R}{p}'$  }
}}}}}}
\UnaryInfC{{\small$ (\globalstateli
,\Br)\transitionKER{r}{\globalstatelj}(\globalstatelf,\Br')$}}
\end{prooftree}
\vspace*{-.5cm}
  \caption{\label{fig:exchange_transition}
  Definition of the relation $\transitionKER{r}{ \protect\globalstatelj}$
 }
\end{figure}


The transition relation $\transitionKER{r}{\globalstatelj}$ in
 Fig.~\ref{fig:exchange_transition} is among abstract configurations of the form
$(\globalstate{l},\Br)$ where $\globalstate{l}$ is a global state of the product
of automata of the studied system and $\Br(p) = (\Crxp{S}{p}, \Crxp{R}{p})$.
Similarly to  function $B$ in \cite{DBLP:conf/fossacs/GiustoLL20}, function $\Br$ allows
to track messages that have a causal link with the unmatched messages that
precede them.
More precisely, we
have:
\begin{align*}
\Crxp{S}{p} =&\{\procofaction{S}{v} \mid v' \cgedgeD{SS} v \mbox{ \& } v' \mbox{
is unmatched } \mbox{ \& } \procofaction{R}{v'} =p \} \\
\Crxp{R}{p} = &\{\procofaction{R}{v} \mid v' \cgedgeD{SS} v \mbox{ \& } v'
\mbox{ is unmatched } \mbox{ \& } \procofaction{R}{v'} = p \mbox{ \& } v \cap R
\neq \emptyset \}
\end{align*}
We denote by $\Br_{\emptyset}$ the initial function $\Br$ where $\Crxp{X}{p} =
\emptyset$ for all $X \in \{S,R\}$ and $p \in \procSet$.
We can, therefore, define a feasible triple, which is, intuitively, a triple that
 corresponds to a \kE{k} runnable by the system.

\begin{definition}[A feasible triple]
For a given system $\system$,
a set composed of a triple of global states $\triple$ and a function $\Br : \procSet \rightarrow (2^{\procSet} \times 2^{\procSet})$  is
 feasible iff there is $m_S \in S^*$ and $m_R \in R^*$ such that
$(\globalstateli,\B_{\emptyset}) \xRightarrow{m_S} (\globalstatelj, \B)
 \xRightarrow{m_R} (\globalstatelf, \B')$
for some $\B, \B'$ and
$(\globalstateli,\Br) \transitionKE{m_S\cdot m_R}{\size{m_S}}
 (\globalstatelf,\Br')$.
\end{definition}

 The following lemma
extends  Lemma~1 in \cite{DBLP:conf/fossacs/GiustoLL20} to ECG with regular
expression.









\begin{lemma}\label{lemma:rcd_cycleSS}
For $r \in \decompsetauto$ and for some $\Br$, $ \ecgraph{r,\Br}$ does not
contains SS cycle iff  for some $\Br'$ $(\globalstateli,\Br)
\transitionKER{r}{\globalstatelj} (\globalstatelf,\Br')$.
\end{lemma}

%\input{proof_lemma_rcd_cycleSS}

We now show that $(\triple, B)$ is feasible if and only if there is a regular
expression $r$ such that $(\globalstateli, \Br)
\transitionKER{r}{\globalstatelj} (\globalstatelf, \Br')$
(Theorem~\ref{theorem:cd_rcd} and \ref{theorem:rcd_cd}).
In the proofs, we will sometimes need to exhibit a candidate word for a given
regular expression without choice operator. We say that $w$ is the
\emph{canonical word} of regular expression $r$ if $w \in \Language{r}$ and $w$
contains two iterations of each star operator in $r$.  For instance, if $r =
\Action{!}{\Message{a}{p}{q}} ( \Action{!?}{\Message{b}{p}{q}} )^*$ then the canonical word is $w =
\Action{!}{\Message{a}{p}{q}}
\Action{!?}{\Message{b}{p}{q}}\Action{!?}{\Message{b}{p}{q}} $.

% \begin{definition}[Canonical word]
% For a given regular expression without choice operator $r$, let $w$ the
% canonical word of $r$ such that $w \in \Language{r}$ and $w$ contains two
% iterations of each star operator.
% \end{definition}
%
%
\begin{theorem}\label{theorem:cd_rcd}
For a system $\system$, for all $\globalstateli, \globalstatelf, B,
B'$, for all sequence of actions $e$ and
$k \in \mathbb{N}$, if
$(\globalstateli,B) \transitionKE{e}{k} (\globalstatelf, B')$ then there is
$\globalstatelj, \Br', r \in \decompsetauto$ and $w \in \Language{r}$
such that $\MSC(e) = \MSC(\func{w}{\varepsilon})$ and $(\globalstateli, B)
\transitionKER{r}{\globalstatelj} (\globalstatelf,\Br')$.
\end{theorem}

%\input{proof_theorem_cd_rcd}

%% {\color{red}REMARK: Est-ce que une preuve si longue est nécessaire ?
%% On a une expression régulière r qui est contenu dans L(SR).
%% On sait que tout mot de L(SR) verifie causal delivery.
%% Donc tout mot de r verifie causal delivey.
%% Si on prend B et $\Br$ égaux, alors si on a rcd, on a cd. }

\begin{theorem}\label{theorem:rcd_cd}
For a system $\system$, for all $\globalstateli,\globalstatelj,
\globalstatelf,\Br,\Br'$, for $r \in \decompsetauto$, if
$(\globalstateli,\Br) \transitionKER{r}{\globalstatelj}
(\globalstatelf,\Br')$ then for all $w \in \Language{r}$ there is $k \in
\mathbb{N}, B'$ such that $(\globalstateli,\Br)
\transitionKE{\func{w}{\varepsilon}}{k} (\globalstatelf,B')$.
\end{theorem}
%\input{proof_theorem_rcd_cd}

\subsection*{Step 4. How to compute $k$}

An exchange can be feasible but not reachable. Indeed, it may happen that the triple is
reachable with a function $\Br$ for which transition
$\xRightarrow[\hspace*{0.1cm}{\scriptstyle \mathsf{rcd}}\hspace*{0.1cm}]{ }$ does not exist.


\begin{definition}[A reachable triple]
  For a system $\system$, a triple $\triple$ is reachable with $\Br$ if
  \begin{itemize}
    \item there is a sequence of triples
    $(\globalstate{l_0}, \globalstate{l_{0'}}, \globalstate{l_1}),
    (\globalstate{l_1}, \globalstate{l_{1'}}, \globalstate{l_2})
    \cdots
    (\globalstate{l_n}, \globalstate{l_{n'}}, \globalstateli)$
    and a function $\Br$ such that
    $(\globalstate{l_0},\Br_{\emptyset})
    \transitionKER{r_0}{\globalstate{l_{0'}}} (\globalstate{l_1}, \Br_1)
    \transitionKER{r_1}{\globalstate{l_{1'}}} (\globalstate{l_2}, \Br_2)
    \cdots
    (\globalstate{l_n}, \Br_n)
    \transitionKER{r_n}{\globalstate{l_{n'}}} (\globalstateli, \Br)$
    with $r_k \in \decompset{k,k',k+1}$;
    \item there is $r \in \decompsetauto$ and $\Br'$ such that
    $(\globalstateli, \Br) \transitionKER{r}{\globalstatelj}
    (\globalstatelf, \Br')$.
  \end{itemize}
\end{definition}


\begin{example}
In the system of Example~\ref{ex:why_decomp}, the triple $((1,0),(1,0),(3,0))$
is feasible as $\LangSRauto \neq \emptyset $ and so $(\globalstateli, \Br)
\transitionKER{r}{\globalstatelj}(\globalstatelf, \Br')$ is verified for
$\Br = ( \Crxp{X}{p} = \emptyset )_{X \in \{S,R\},p \in \procSet, }$ and $r =
\Action{!?}{\Message{b}{p}{q}} \Action{!}{\Message{c}{p}{q}}$.
However, the global state $(1,0)$ is reachable only if message $a$ is sent but
not received. As a consequence, in $\Br$, $\Crxp{S}{q} = \{p\}$.
With this condition,
there is no $(\globalstatelf, \Br')$ such that
$(\globalstateli, \Br)
\transitionKER{r}{\globalstatelj}(\globalstatelf, \Br')$ for $r =
\Action{!?}{\Message{b}{p}{q}} \Action{!}{\Message{c}{p}{q}}$ because of the
edge $b \cgedgeD{SS} \lambdanode_q$ added with rule (4) in the definition of the
extended conflict graph. This edge allows to add $ q \in \Crxp{R}{q}'$, and so
the relation transition is not verified.
\end{example}

So, we can define the set of exchanges
runnable when the triple is reachable:
\begin{align*}
  \decompreachsetauto = \{  r \mid  & ~ r \in \decompsetauto, \triple
    \mbox{ is reachable with }\Br,  \\
    & \mbox{ and } (\globalstateli, \Br) \transitionKER{r}{\globalstatelj}
      (\globalstatelf,\Br') \mbox{ for some }\Br'\}
\end{align*}

%\paragraph*{Step 5. How to compute $k$}
Once we have computed the set of reachable triples, we have all the necessary
information to estimate a candidate for \kSity{k}. The size of a triple is
linked to the size of the SCC of its conflict graph. Hence, since SCCs represent
messages that depend on each other, the size of the biggest SCC determines the
size of the exchange.  Now, if the SCC contains an edge labelled with $\star$ {\color{red}commentaire post-soumission : typo} it
means that a part of the graph can be repeated and thus the exchange can grow
arbitrarily. In such case (see Example~\ref{exmp:large_exchange} below) we say that the triple has
size $k = \infty$.

\begin{definition}[Size of a triple]\label{def:size_triple}
Let $\triple$  be a triple reachable with $\Br$, $r \in \decompreachsetauto$
such that $(\globalstate{l_i},\Br) \transitionKER{r}{\globalstate{l_j}}
(\globalstate{l_f}, \Br')$ for some $\Br'$ and
$SC$ the set of SCC of $\scgraph{r}$.
The size of $r$ is defined by:

$\size{r} = \left\{
	\begin{array}{ll}
		\infty & \mbox{ if } v \cgedgeS v \in	SCC \mbox{ for some } SCC \in SC \\
		max_{SCC \in SC} \size{SCC} & \mbox{ otherwise }
	\end{array}
\right.
$
The size of $\triple$ is:

$ \size{\triple} = \{ max(\size{r}) \mid r \in \decompsetauto \}$
  with $\infty > n, \forall n \in \mathbb{N}$.
%$r$, resp. $\triple$, is \emph{arbitrarily large} if
%$\size{r} = \infty$, resp. $\size{\triple} = \infty$.
\end{definition}

\begin{example}[Exchange with an arbitrarily large size]\label{exmp:large_exchange}
\input{exmp_large_exchange.tex}
\end{example}

Next theorem shows that our construction is correct, if a regular expression has finite size $k$ than all words in the language have SCCs of size at most $k$. We first need an auxiliary definition:

% Considering conflict graph without star edges, if some messages form an SCC then
% they all depend on each other and they have to be in the same exchange. If a
% message is not in the SCC then it can be done in an other exchange. In the same
% way, if the conflict graph is composed of several SCC, each of them can be done
% in a separated exchange. Therefore, the size of the biggest SCC in the conflict
% graph determines the size of the exchange.

\begin{definition}[Size of an exchange]
  Let $e = e_1 \cdot e_2 \cdots e_n$ be an exchange. The size of $e$ is define
  by: $\size{e} = \size{SCC}$ where $SCC$ is the biggest SCC belonging to
  $\cgraph{e}$.
\end{definition}



\begin{theorem}\label{theorem:k_bound}
  For $r$ a regular expression without choice operator, $\size{r} = k \neq \infty$
if and only if for all $w \in \Language{r}$, all SCC in
$\cgraph{\func{w}{\varepsilon}}$ are of size at most $k$.
\end{theorem}

%\input{proof_theorem_k_bound}

If a system contains one reachable triple of size $ k = \infty$,
then the system is not \kSable{k}.



\begin{theorem}\label{theorem:large_not_ksynchro}
For a given system $\system$, if there is a reachable triple $\triple$ such that
there exists $r \in \decompreachsetauto$  such that $\size{r} = \infty$
then $\system$ is not \kSable{k} for any $k$.
\end{theorem}
%\input{proof_theorem_large_not_ksynchro}

Finally, if all exchanges are of finite size then the largest one is a candidate
for \kSity{k}.
%
% \begin{lemma}\label{lemma:k_max}
%   For a system $\system$ and a triple $\triple$, if $\size{\triple} = k \neq
%   \infty$ then there is no exchange $e = e_S \cdot e_R$, $e_S \in S^*, e_R \in
%   R^*$, such that $ \size{e} > k$ and  $\globalstate{l_0} \Rightarrow^*
%   \globalstate{l_i} \xRightarrow{e_S} \globalstate{l_j} \xRightarrow{e_R}
%   \globalstate{l_f}$.
% \end{lemma}
%
% \begin{proof}
%   Let $\triple$ be a triple such that $\size{\triple} = k$.
%   By contradiction, suppose that there is an exchange $e = e_S \cdot e_R$, $e_S
% \in S^*, e_R \in R^*$, such that $ \size{e} > k$ and  $\globalstate{l_0}
% \Rightarrow^* \globalstate{l_i} \xRightarrow{e_S} \globalstate{l_j}
% \xRightarrow{e_R} \globalstate{l_f}$.
%
%   As $e$ is an exchange over $\triple$, then we have $(\globalstate{l_i}, B)
%   \transitionKE{e}{n} (\globalstate{l_f},B')$ for some $B,B'$. Therefore, by
%   Theorem~\ref{theorem:cd_rcd}, there is $r \in \decompset{i,j,f}$ and $w \in
%   \Language{r}$ such that $MSC(e) = MSC(\func{w}{\varepsilon})$ and
%   $(\globalstate{l_i}, \Br) \transitionKER{r}{\globalstate{l_j}}
%   (\globalstate{l_f}, \Br')$. More, as $e$ is runnable by the system, there is
%   $\Br$ such that $\triple$ is reachable and $(\globalstate{l_i}, \Br)
%   \transitionKER{r}{\globalstate{l_j}} (\globalstate{l_f}, \Br')$, therefore, $r
%   \in \decompreachset{i,j,f}$
%
%   The size of $r$ is taken into account to evaluate the size of $\triple$.
%  \begin{itemize}
%    \item Either there is $v,v'$ such that $v \cgedge{\star} v' \cgedge{}^* v \in
%    \scgraph{r}$. Then, $\size{r} = \infty$ and $\size{\triple} = \infty $, which
%    is a contradiction.
%    \item Or there is no cycle with a star edge in $\scgraph{r}$. The size of $r$
%    corresponds to the biggest SCC in $\scgraph{r}$, denoted $SCC_r$, which does
%    not contains star edge since $\size{r} \neq \infty$. $w \in \Language{r}$ so
%    the biggest SCC of $\cgraph{\func{w}{\varepsilon}} = \cgraph{e}$, denoted
%    $SCC_e$ is the same as $SCC_r$, messages in it being necessarily contained in
%    $w$ since $SCC_r$ does not contain a star edge (allowing messages to be
%    omitted). Then $\size{e} = \size{r}$. Finally, $\size{\triple} \geq \size{r}$
%    and so $\size{\triple} \geq \size{e}$ which is a contradiction and concludes
%    this proof.
%  \end{itemize}
% \end{proof}

\subsection*{Step 5. Borderline violations}
Once we have determined with previous steps a candidate for $k$, we still have
to check if there are borderline violations.

\begin{definition}[Borderline violation]
 %Let $\system$ be a non \kSable{k} system.
 A non \kSable{k} execution $e$
 %\in\asEx(\system)$
 is a borderline violation if $e=e'\cdot r$, $r$ is a reception and  $e'$ is \kSable{k}.
\end{definition}


Indeed, if a system is not \kSable{k}, then there is a borderline violation, \ie
an execution that is not \kSable{k} but becomes \kSable{k} if we ignore the last
reception.  As next example shows, some borderline
violations are not detected by our procedure.


%
% Still, some borderline violations (see \cite{DBLP:conf/fossacs/GiustoLL20}, Def. 8)
% are not detected. To this aim, by means of algorithm, we verify if the system is
% \kSable{k} for this $k$.
% Indeed, an execution  which is not in the form
% of an exchange will not be seen by our analysis. Therefore, a borderline violation
% of this form will not be caught.

\begin{example}
\input{exmp_borderline.tex}
\end{example}

Algorithm $synchronizable(\system)$ (Algo.~\ref{algo:synchro} and \ref{algo:test}) sums up all the
steps described so far. $Gstates$ collects the reachable global states that have
to be analyzed and function $test$ verified that $(\globalstateli, \Br)
\transitionKER{r}{\globalstatelj} (\globalstatelf, \Br')$ for some $r$.
The algorithm in
\cite{DBLP:conf/fossacs/GiustoLL20}  that checks if a system is \kSable{k} for a $k$
is noted as $kSynchronizable(\system,k)$.
Finally,
we can state our main result.

\begin{theorem}\label{theorem:algo}
  A given system $\system$ is \kSable{k} iff $synchronizable(\system) = k'$
  and $kSynchronizable(\system,k') = True$ with $k' < \infty$.
\end{theorem}
%\input{proof_theorem_algo}
\begin{remark}
  The resulting $k$ is the smallest that we can find. Indeed, if the system is
  \kSable{k} then there is no $k' < k$ such that the system is also \kSable{k'}.
  All exchanges that we have  analysed are runnable by the system, hence, if a $k$
  is taken into account then it can not be ignored.
\end{remark}
% \begin{lemma}
% Let $\system$ be a system and $k = max ( \size{\triple})_{\triple \in \Gamma}$.
% If $\system$ is not \kSable{k} then there is no $k' > k$ such that $\system$ is
% \kSable{k'}.
% \end{lemma}
%
% To resume, following algorithm $Synchronizable(\system)$ wrote in pseudo-code
% describes all the approach. Let suppose function $kSynchronizable(\system,k)$
% designates the function that returns $true$ if $\system$ is \kSable{k} for a given
% $k$. A global state is added to $gstates$ to be visited with a function $\Br$.
% By default, the value of $visited$ is $false$.
% In function $test$, we add $(\globalstate{l_f}, \Br')$ to $gstates$ such that
% $(\globalstate{l_i}, \Br) \transitionKER{r}{\globalstate{l_j}}
% (\globalstate{l_f},\Br')$.

\begin{algorithm}\label{algo:synchro}
\SetAlgoLined
\DontPrintSemicolon
\SetKwProg{Fn}{Function}{}{end}
\Fn{synchronizable($\system$) : integer}{
	$gstates = \{(\globalstate{l_0}, \Br_{\emptyset})\}$ \;
	$k = 0$ \;
  \For{$(\globalstateli, \Br)$ in $gstates$}{
		\If{$!~(\globalstateli, \Br).visited$}{
			$(\globalstateli, \Br).visited = true$\;
			\For{$\globalstatelj, \globalstatelf$ in $\prod _{p\in \procSet} L_p$}{
				\If{$test(\globalstateli,\globalstatelj, \globalstatelf, \Br) \geq 0$}{
					$k = max (test(\globalstateli,\globalstatelj, \globalstatelf, \Br), k)$	\;
				}
				\Else{
					\Return $-1$
				}
			}
		}
	}
\Return $k$
}
\caption{Return a candidate $k$}
\end{algorithm}


\begin{algorithm}\label{algo:test}
\SetAlgoLined
\DontPrintSemicolon
\SetKwProg{Fn}{Function}{}{end}

\Fn{$test(\globalstateli, \globalstatelj, \globalstatelf, \Br)$ : integer}{
			%Langage d'envoi et de reception
			build $\LangSauto$\;
			build $\LangRauto$\;
			\If{$\LangSauto \neq \emptyset$ and $\LangRauto \neq \emptyset$}{
				%Langage envoi et reception combines
				build $\LangSRauto$\;
				\If{$\LangSRauto \neq \emptyset$}{
					%Contruction des decompositions
					build $\decompsetauto$ \;
					k = 0 \;
					\For{$r \in \decompsetauto$}{
						%Pour chaque chemin, est-il causal delivery ?
            build $\ecgraph{r, \Br}$\;
              \If{ $!(\exists v$ s.t. $v \cgedgeD{SS} v \in \ecgraph{r, \Br})$}{
                % Si on trouve un chemin causal et que l'état final n'est pas déjà dans les etats atteignables, on l'ajoute
  							\If{$!( (\globalstatelf,\Br')$ in $gstates)$}{
  								$gstates.add(\globalstatelf, \Br')$\;
  							}
                build $\scgraph{r}$\;
                \If{$\exists v,v'$ s.t. $v\cgedgeS v'\cgedge{}^*v \in \scgraph{r}$}{
                %Taille arbitrairement grande
                  \Return ~-1\;
                }
                %Sinon on conserve la taille
                \Else{
                $k = max (k, \size{ r })$}
              }
					}
				}
        \Else{\Return 0}
			}
      \Else{\Return 0}
			}
      \Return k\;
      \caption{Return the size of a triple}
\end{algorithm}


==> exmp_borderline.tex <==
Let $\system_2$ on Fig.~\ref{fig:borderline}(a) a system.
The computed candidate for \kSity{k} is $k =1$.
Indeed, all exchanges of the system have independent messages, like MSC in Fig.~\ref{fig:borderline}(b) and its conflict graph in Fig.~\ref{fig:borderline}(c).

However, MSC in   Fig.~\ref{fig:borderline}(d) shows an execution runnable by $\system_2$ which is a borderline violation but which is not an exchange. Indeed, it cannot be divided into \kE{k} but becomes \kSable{1} with the deletion of the reception of $\amessage_1$.
This execution is not considered by our approach because of the reception of $\amessage_2$ that have to be done before the send of $\amessage_3$ which ignore all executions where $\amessage_2$ and $\amessage_3$ are in the same \kE{k}.
 %
 % that is not \kSable{k}, and the MSC on Fig.~\ref{fig:msc_borderline}
 % representing a borderline violation of its system as it cannot be divided into
 % \kE{k}s and the deletion of reception of $\amessage_1$ makes it divisible.
 % Indeed, by looking for executions that can be divided by \kE{k}s, messages
 % $\amessage_1$ and $\amessage_3$ will never be sent in the same sequence because
 % of $\amessage_2$ that have to be sent and received between these two sends.
 % Therefore, executions depicted by the MSC are not considered.

\begin{figure}[t]\label{fig:borderline}
%\begin{minipage}[c]{.60\linewidth}
%\centering
\begin{center}
\input{borderline_msc.tex}
%\end{minipage}
%\begin{minipage}[c]{.37\linewidth}
%\begin{center}
%\input{borderline_system.tex}
\end{center}
%\end{minipage}
\caption{\textbf{(a)}: MSC of a borderline violation of $\system_2$, \textbf{(b)}: System $\system_2$ }
\end{figure}


==> exmp_build_conflict_graph.tex <==
% !TEX root = vmcai.tex
 For $exp =
( \Action{!?}{\Message{a}{q}{r}}
(\Action{!?}{\Message{b}{p}{r}} )^*
\Action{!?}{\Message{c}{q}{r}})^*
\Action{!}{\Message{d}{p}{r}}$
(information on senders and receivers will be omitted to increase readability):
we give the encoding of the projections of the transformed regular expression and  the final conflict graph (Fig. \ref{fig:exmp:cgraph}).
$$
\begin{array}{ll}
\transf{exp} =&((!?a_0 (!?b_0 \dotstar !?b_1) !?c_0)  \dotstar (!?a_1 (!?b_2
\dotstar !?b_3) !?c_1) ) !d_0 \\

t(exp) \proj{pS} = & ((b_0 \dotstar b_1)\dotstar
(b_2 \dotstar b_3)) d_0\\

\encode{t(exp) \proj{pS}} =&  (\{b_0,b_1,b_2,b_3,d_0\},\{ b_0 \cgedgeS
b_1, b_2 \cgedgeS b_3, b_3 \cgedge{SS} d_0 \}, b_0,d_0)\\

\transf{exp} \proj{qS} = &(a_0  c_0 \dotstar a_1 c_1 )\\

\encode{\transf{exp} \proj{qS}} =& (\{a_0,c_0,a_1,c_1\}, \{ a_0 \cgedge{SS} c_0
, a_1
\cgedge{SS} c_1, c_0 \cgedgeS a_1\}, a_0, c_1)\\

\transf{exp} \proj{rR} = & (a_0 (b_0 \dotstar b_1) c_0)  \dotstar (a_1 (b_2
\dotstar b_3) c_1)\\


\encode{exp \proj{rR} } =& (\{b_0,b_1,a_0,c_0,b_2,b_3,a_1,c_1\},  \{ b_0
\cgedgeS b_1 , a_0 \cgedge{RR} b_0, b_1\cgedge{RR}c_0, b_2 \cgedgeS
b_3 ,\\
& \qquad  a_1 \cgedge{RR} b_2, b_3\cgedge{RR}c_1 , c_0 \cgedgeS a_1 \},
a_0, c_1) \\

\end{array}
$$






\begin{figure}[t]
\begin{center}

\begin{tikzpicture}
	\node[draw] (a0) at (0,0) {$a_0$};
	\node[draw] (a1) at (6,-2) {$a_1$};
	\node[draw] (b0) at (2,0) {$b_0$};
	\node[draw] (b1) at (4,0) {$b_1$};
	\node[draw] (b2) at (4,-2) {$b_2$};
	\node[draw] (b3) at (2,-2) {$b_3$};
	\node[draw] (c0) at (6,0) {$c_0$};
	\node[draw] (c1) at (0,-2) {$c_1$};
	\node[draw] (d) at (-2,-2) {$d_0$};


	\draw[->] (a0) to node[midway, above]{RR} (b0);
	\draw[->] (b0) to node[midway, above]{$\circledast$} (b1);
	\draw[->] (b1) to node[midway, above]{RR} (c0);
	\draw[->] (c0) to node[midway, right]{$\circledast$} (a1);
	\draw[->] (a1) to node[midway, above]{RR} (b2);
	\draw[->] (b2) to node[midway, above]{$\circledast$} (b3);
	\draw[->] (b3) to node[midway, above]{RR} (c1);
	%\draw[->] (c1) to node[midway, above]{RR} (d);

	\draw[->] (a0) to[bend left=40] node[midway, above]{SS} (c0);
	\draw[->] (a1) to[bend left=40] node[midway, below]{SS} (c1);
	\draw[->] (b3) to[bend left = 40]  node[midway, below]{SS} (d);

%	\draw[->, dashed] (a0) to node[midway, above, sloped]{SS} (a1);
%	\draw[->, dashed] (a0) to node[midway, above, sloped]{SS} (b3);
%	\draw[->, dashed] (a0) to node[midway, above, sloped]{SS} (c1);
%		\draw[->, dashed] (a0) to node[midway, above, sloped]{SS} (d);

\end{tikzpicture}

\end{center}
\label{fig:exmp:cgraph}
\caption{The conflict graph of Example \ref{ex:cgfromregexp} }
\end{figure}


==> exmp_large_exchange.tex <==

System $\system$ is depicted in Fig.~\ref{fig:large_msc}(e) and let triple $t =
((0,0,0),(1,0,1),(1,1,2))$.
For this triple,
we have $$\LangSRauto =~
\Action{!?}{\Message{a}{p}{r}} (\Action{!?}{\Message{b}{p}{q}})^*
\Action{!?}{\Message{c}{r}{q}} (\Action{!}{\Message{b}{p}{q}})^* ~ + ~
\Action{!?}{\Message{c}{r}{q}} \Action{!?}{\Message{a}{p}{r}}
(\Action{!?}{\Message{b}{p}{q}})^* $$
Then,
\begin{align*}
  \decompset{init,mid,final} = \{ &
  \Action{!?}{\Message{a}{p}{r}} \Action{!?}{\Message{c}{r}{q}},
  \Action{!?}{\Message{a}{p}{r}} (\Action{!?}{\Message{b}{p}{q}})^*
  \Action{!?}{\Message{c}{r}{q}}, \\
&  \Action{!?}{\Message{a}{p}{r}}
  \Action{!?}{\Message{c}{r}{q}} (\Action{!}{\Message{b}{p}{q}})^*,
  \Action{!?}{\Message{a}{p}{r}} (\Action{!?}{\Message{b}{p}{q}})^*
  \Action{!?}{\Message{c}{r}{q}} (\Action{!}{\Message{b}{p}{q}})^*, \\
&   \Action{!?}{\Message{c}{r}{q}} \Action{!?}{\Message{a}{p}{r}}, 
  \Action{!?}{\Message{c}{r}{q}} \Action{!?}{\Message{a}{p}{r}}
  (\Action{!?}{\Message{b}{p}{q}})^*
  \}
\end{align*}
Consider $r= \Action{!?}{\Message{a}{p}{r}}
(\Action{!?}{\Message{b}{p}{q}})^* \Action{!?}{\Message{c}{r}{q}} \in
\decompset{init,mid,final}$ and its conflict graph which is depicted in
Fig.~\ref{fig:large_msc}(d). As we can see, we have a star edge included in a
cycle.
MSCs in Fig.~\ref{fig:large_msc} (a), (b) and (c) give an example on how th
exchange can grow. This means that we can build \kE{k}s of arbitrarily large
size. As consequence, there is no $k$ such that $\system$ is \kSable{k}.

\begin{figure}[t]
\begin{center}
\input{large_msc.tex}
\input{large_system.tex}
\caption{\textbf{(a)}, \textbf{(b)} and \textbf{(c)} depict MSCc runnable by
$\system_1$, \textbf{(d)} is $\scgraph{\Action{!?}{\Message{a}{p}{r}}
(\Action{!?}{\Message{b}{p}{q}})^* \Action{!?}{\Message{c}{r}{q}}}$,
\textbf{(e)} system $\system$}
\label{fig:large_msc}
\end{center}
\end{figure}


==> lemma-soundness-alpha-automaton.tex <==
\begin{proof}
Let $w\in\Sigma^*$ and $\dag\Message{\amessage}{p}{q}$ be fixed.
Let $G_1=\pgraphof{msc(w)}$ and $G_2=\pgraphof{msc(w\cdot\dag\Message{\amessage}{p}{q})}$
and let us compare $G_1$ and $G_2$. First, there is an extra vertex $v_0$
in $G_2$ that represents $\dag\Message{\amessage}{p}{q}$, with
$\lambda_S(v_0)=\{p\}$ and either $\lambda_R(v_0)=\{q\}$ (if $\dag=!?$)
or $\lambda_R(v_0)=\emptyset$ (if $\dag=?$).
Now, consider the extra edges. Obviously, these extra edges have
$v_0$ either as source or as destination. First consider the edges
with $v_0$ as destination. The send event of $v_0$ happens after
all send events of $p$, so for all $v\neq v_0$ such that $p\in\lambda_S(v)$,
$(v,v_0)\in E_2$.
In the case where $\dag=!?$, the receive event of $v_0$ also happens
after all send and receive events of $q$, so for all
$v\neq v_0$ such that $q\in\lambda_S(v)\cup\lambda_R(v)$, $(v,v_0)\in E_2$.
There are no
other incoming edges in $v_0$
Now, consider the outgoing edges of $v_0$. The send event of $v_0$ happens
before all receive events of $p$, so for all
$v\neq v_0$ such that $p\in\lambda_R(v)$, $(v_0,v)\in E_2$.
To sum up, we have:


$$
\begin{array}{lll}
E_2&=&E_1\cup\{(v,v_0)\mid p\in\lambda_S(v)\}\\
&\cup&\{(v_0,v)\mid p\in\lambda_R(v)\}\\
&\cup&\left\{\begin{array}{ll}
\{(v,v_0)\mid q\in\lambda_S(v)\cup\lambda_R(v)\} & \mbox{if }\dag=!?\\
\emptyset & \mbox{if }\dag=!
\end{array}\right.
\end{array}
$$

Observe now that the rules to add vertices and edges to go from $G_1$
to $G_2$ are exactly the same as the rules to go from $G$ to $G'$
in the definition of $\delta_g(G,\dag\Message{\amessage}{p}{q})$.
Assume that $G=\alpha(G_1)=\alpha(\pgraphof{msc(w)}$.
Then $G'$ is a partial abstraction of $G_2$. So by the discussion above,
$$\alpha(G')=\alpha(G_2).$$
Now, by definition of $\delta_g$,
$\delta_g(G,\dag\Message{\amessage}{p}{q}))=\alpha(G')$.
To sum up
$$
\delta_g(G,\dag\Message{\amessage}{p}{q})
=\alpha(G_2)=\alpha(\pgraphof{msc(w\cdot\dag\Message{\amessage}{p}{q})}).
$$
\qed
\end{proof}


==> pour-memoire.tex <==
\section{Things to include somewhere or remove}

A formal definition of the ``layout'' reached after
a MSC $\mu$ could be the Nerode equivalence class of $\mu$ with respect
to $\asTr(\system)$ in the monoid of MSC concatenation (we omit details for readability). For now, let us say that the
layout at the end of MSC $\mu$ is a pair
$(\globalstate{l},\Br)$
where $\globalstate{l}$ is the global state reached at the end of $\msc$,
and $\Br:\procSet\to 2^{\procSet}\times2^{\procSet}$ is a summary
about when and how unmatched messages were sent during $\msc$.
A first, simpler, intuition is that this summary gathers the information
for each buffer whether it contains an unmatched message.

\noindent
\begin{minipage}[c]{10cm}
This intuition however is too simple, and it is actually
necessary to remember which process sent an unmatched message in this buffer, and which other processes are causally
after this unmatched message. The example MSC on the right illustrates the subtleties behind the scene. The first message $\amessage_1$ is
unmatched, but still the message $\amessage_3$ is matched. Indeed, $\amessage_1$ does not necessarily happen
before $\amessage_3$ even if it appears before in the concatenation. Actually, this MSC corresponds to a valid
execution where $\amessage_3$ is sent before $\amessage_1$.
\end{minipage}
\begin{minipage}[c]{3cm}
	\hspace*{0.5cm}
\begin{tikzpicture}[baseline]
		\draw (0,0) to (0,-3.5) ;
		\draw (1,0) to (1,-3.5) ;
		\draw (2,0) to (2,-3.5) ;
		\draw (0,0.25) node{$p$} ;
		\draw (1,0.25) node{$q$} ;
		\draw (2,0.25) node{$r$} ;
		\draw[->,>=latex] (0,-1) to node [above, pos = 0.9] {$\amessage_1$} (.5,-1);
		\draw[->,>=latex,dashed] (.5,-1) to (1,-1);
		\draw[->,>=latex] (1,-2) to node [above] {$\amessage_2$} (0,-2);
		\draw[->,>=latex] (2,-3) to node [above] {$\amessage_3$} (1,-3);
                \draw[dashed] (-0.5,-1.5) -- (2.5,-1.5);
                \draw[dashed] (-0.5,-2.5) -- (2.5,-2.5);
\end{tikzpicture}
\end{minipage}

This complication will be later discussed, but it is enough for now to
understand that
the function $\Br:\procSet\to 2^{\procSet}\times2^{\procSet}$ deals with
unmatched messages.
We write
$(\globalstate{l},\Br)\transitionfeas{\msc}(\globalstate{l'},\Br')$
to denote that, if it starts in the layout
$(\globalstate{l},\Br)$, the system may execute $\msc$ and
end in the layout $(\globalstate{l'},\Br')$.
We also write $(\globalstate{l_0},\Br_0)$ to denote the initial layout.


==> proof-lem-b-automaton-soundness.tex <==
\begin{proof}
\begin{itemize}
\item[$\Rightarrow$]
Let $\Br^{(0)}$, $\Br^{(1)}$ and $w$ be fixed such that
$\Br^{(0)}\Tr{w}\Br^{(1)}$, and 
let us prove that $\Br^{(0)}\Tr{msc(w)}\Br^{(1)}$.
We reason by induction on the length of $w$. The case $w=\epsilon$ is 
immediate. Let us assume $w=ua$, and let us assume by induction
hypothesis that there is some $\Br$ such that $\Br^{(0)}\Tr{u}\Br$
and $\Br^{(0)}\Tr{msc(u)}\Br$.
\item[$\Leftarrow$]
\end{itemize}
\end{proof}


==> proof_lemma_Aut_SR.tex <==
\begin{quote}
{\bf Lemma 2}
For $e = s_1 \cdots s_n \cdot r_1 \cdots r_{n'}$ with $s_1 \cdots s_n \in S^*$
and  $r_1 \cdots r_{n'} \in R^*$, if there is a triple $\triple$ and $ \B, \B'$
such that $$(\globalstateli, \B_{\emptyset}) \xRightarrow{s_1 \cdots s_n}
(\globalstatelj, \B) \xRightarrow{r_1 \cdots r_{n'}} (\globalstatelf,
\B')$$ then there is $w \in \Language{\AutSRauto}$ such that $\MSC(e) =
\MSC(\func{w}{\varepsilon})$.\end{quote}

\begin{proof}
Let $e = s_1 \cdots s_n \cdot r_1 \cdots r_{n'}$ such that $s_1 \cdots s_n \in
S^*$ and  $r_1 \cdots r_{n'} \in R^*$, and for a triple $\triple$ and $ \B,
\B'$, $(\globalstateli, \B_{\emptyset}) \xRightarrow{s_1 \cdots s_n}
(\globalstatelj, \B) \xRightarrow{r_1 \cdots r_{n'}} (\globalstatelf,
\B')$.

Let  $e' = s_1 \cdots s_n \cdot r'_1 \cdots r'_{n'}$ be a linearization of
$\MSC(e)$ where the order of sends $s_1 \cdots s_n$ is the same as in $e$ and
where receptions $r'_1 \cdots r'_{n'}$ follow the same order as the sends. These
permutations are possible as:
\begin{itemize}
\item either two messages are causally related then the mailbox
communication implies that their reception are already in the same order,
\item or they are not, in which case there is no
order imposed by the communication on the receptions and all permutations are
possible.
\end{itemize}

We define $w$ a sequence of matched and unmatched sends as follows:
$$w = g(s_1 \cdots s_n \cdot r'_1 \cdots r'_{n'}) =  \left\{
	\begin{array}{l l}
		!?s_1 \cdot g(s_2 \cdots s_n \cdot r'_2 \cdots r'_{n'})
      &\mbox{ if } s_1 \matches r'_1  \\
		!s_1 \cdot g(s_2 \cdots s_n \cdot r'_1 \cdots r'_{n'})& \mbox{ otherwise }
	\end{array}
\right.
$$


We prove that $(\globalstate{l_0}, \emptyset ) \xRightarrow{w} (\globalstate{l},
\condemned)$ by induction on the length of $w$.
\begin{enumerate}
  \item[\textnormal{BASE}]
    $w = \varepsilon$, the case is immediate;
  \item[\textnormal{REC}]
    $w = a_1 \cdots a_n$, we know by induction that $(\globalstate{l_0}, \empty)
    \xRightarrow{a_1 \cdots a_{n-1}} (\globalstate{l}, \condemned)$. We prove
    that $(\globalstate{l}, \condemned) \xrightarrow{a_n} (\globalstate{l'},
    \condemned')$.
    \begin{itemize}
      \item if $a_n = !\Message{\amessage}{p}{q}$ then, since $s_1 \cdots s_n$
      is a prefix of a word in $\LangSauto$, the arc exists by construction.
      Thus, $(\globalstate{l}, \condemned) \xrightarrow{a_n} (\globalstate{l'},
      \condemned \cup \{q\})$.
      \item if $a_n = \Action{!?}{\Message{\amessage}{p}{q}}$ and
      $\globalstate{l} = \globalstate{l}_{m_S,m_R}$, since $s_1 \cdots s_n$ is
      a prefix of a word in $\LangSauto$ then $\globalstate{l_{m_S}}
      \xrightarrow{\send{p}{q}{\amessage}} \globalstate{l_{m'_S}} \in
      \delta_{\AutSauto}$ . Since $r_1 \cdots r_{n'}$ is a prefix of a word in
      $\LangRauto$ then $\globalstate{l_{m_R}}
      \xrightarrow{\rec{p}{q}{\amessage}} \globalstate{l_{m'_R}} \in
      \delta_{\AutRauto}$.
      Since $e$ is an execution, it is not possible that $e' =
      \send{p'}{q}{\amessage'} \cdots$ $ \send{p}{q}{\amessage} \cdots $ $
      \rec{p}{q}{\amessage}$ for any linearization $e'$ of $MSC(e)$ where $e'$
      keeps the order on send actions.  Then $q \notin \condemned$ and so
      $(\globalstate{l}, \condemned) \xrightarrow{a_n} (\globalstate{l'},
      \condemned)$.
    \end{itemize}
\end{enumerate}

Therefore, for $\globalstate{l} = \globalstate{l}_{m_S,m_R}$, as $s_1\cdots s_n
\in \LangSauto$ then we have $\globalstate{l}_{m_S} \in F_{\AutSauto}$. As $r_1\cdots
r_{n'} \in \LangRauto$ then $\globalstate{l}_{m_R} \in F_{\AutRauto}$, and so,
$\globalstate{l} \in F_{\AutSRauto}$.
%
Finally, there is $(\globalstate{l_0}, \emptyset )
\xRightarrow{w} (\globalstate{l}, \condemned)$ and $\globalstate{l} \in
F_{\AutSRauto}$ so  $w \in \Language{\AutSRauto}$.
\qed
% Now, by contradiction, assume that $ w \notin \LangSRauto$. Then there is
% no path from the initial state to a final state $\globalstate{l}_{m,m'}$
% reachable with $w$. As  $\globalstate{l}_{m,m'}$ is not reachable:
% \begin{itemize}
% \item either not all the sends are done: but $s_1 \cdots s_n \in \LangSauto$ by
% construction of $\AutSauto$,  and there is a send transition corresponding of
% each send transition of $\AutSauto$ in
% $\AutSRauto$;
% \item or not all the receptions are done:
% \begin{itemize}
% \item either a reception is not available in $\AutRauto$: because of the
% mailbox communication, messages with a causal dependency  have to be received in
% the same order as they have been sent; otherwise they have no causal dependency
% and the automaton $\AutRauto$ contains all permutations of receptions and in
% particular $r'_1 \cdot r'_{n'}$. Then, as $r'_1 \cdots r'_{n'}$ is a
% linearization of $\MSC(e)$, $r'_1 \cdots r'_{n'} \in  \LangRauto$.
% \item  or a matched send transition is not available: $e$ verifies causal
% delivery, so all linearizations of $\MSC(e)$ verify causal delivery, in
% particular $e'$. As $e'$ verifies causal delivery, for each reception, the
% concerned process is not forbidden and the reception can be done.
% \end{itemize}
% \end{itemize}
%
% As each case leads to a contradiction, then there is a path from the initial
% state to $\globalstate{l}_{m,m'}$ with $w$ and so $w \in \LangSRauto$.

\end{proof}


==> proof_lemma_SR_D.tex <==
\begin{quote}
{\bf Lemma 3}
 $r \equiv \decomp{r}$.
\end{quote}

\begin{proof}
   By induction on $r$:
  \begin{description}
    \item[\textnormal{BASE}] Trivial.
    \item[\textnormal{REC}]
    \begin{itemize}
      \item If $ r= r_1 \cdot r_2$, by inductive hypothesis, we have $r_1 \equiv
      \decomp{r_1}$ and $r_2 \equiv \decomp{r_2}$.
      $w \in r_1\cdot r_2$ if and only if $w = w_1 \cdot w_2$ such that
      $w_1\in r_1$ and $w_2 \in r_2$.
      That is equivalent to have $w_1 \in \decomp{r_1}$ and $w_2 \in \decomp{r_2}$. Finally,
      $\exists i,j, w_1 \in r_1^i, w_2 \in r_2^j$ if and only if $w \in \decomp{r_1 \cdot r_2}$.
      \item If $r = r_1 +r_2$, by inductive hypothesis, we have $r_1 \equiv
      \decomp{r_1}$ and $r_2 \equiv \decomp{r_2}$.
      By definition, $r \equiv \decomp{r_1} + \decomp{r_2} \equiv \decomp{r_1 + r_2}$.
      \item If $r = r_1^*$, by inductive hypothesis, we have $r_1 \equiv \decomp{r_1}$.
      Observe that $$(r_1^1 + \cdots + r_1^n)^* \equiv ((r_1^1)^* \cdots
      (r_1^n)^* )^*$$ Moreover, for all $I \subseteq \decomp{r_1}$,
      $(\bullet_{r_1^i \in I} (r_1^i)^* )^* \subseteq ((r_1^1)^* \cdots
      (r_1^n)^* )^*$ and so $$((r_1^1)^* \cdots (r_1^n)^* )^* \equiv \sum_{I
      \in 2^{\decomp{r_1}}} (\bullet_{r_1^i \in I} (r_1^i)^* )^* \equiv
      \decomp{r_1^*} $$\qed
    \end{itemize}
  \end{description}
\end{proof}


==> proof_lemma_SR_causal.tex <==
\begin{quote}
{\bf Lemma 1}
For a system $\system$ and a triple $\triple$, if $w \in \LangSRauto$ then
$MSC(\func{w}{\varepsilon})$ satisfies causal delivery. 
\end{quote}

\begin{proof}
Let $\system$ be a system, $\triple$ be a triple of global states and $w \in
\LangSRauto$. $\func{w}{\varepsilon}$ is a linearization of the partial order of
$MSC(\func{w}{\varepsilon})$. For all $i,j$ such that $a_i \prec a_j $, $a_i =
\send{p}{q}{\amessage} \in \func{w}{\varepsilon}$ and $a_j =
\send{p'}{q}{\amessage'} \in \func{w}{\varepsilon}$.
\begin{itemize}
  \item If $\exists i',j'$ such that $a_i \matches a_{i'}$ and $a_j \matches
  a_{j'}$ then, by construction of $\func{w}{\varepsilon}$ from $w$, we have
  $a_{i'} \prec a_{j'}$.
  \item If $\nexists i'$ such that $a_i \matches a_{i'}$, as $w \in \LangSRauto$
  and by construction of automaton $\AutSRauto$, the transition corresponding to
  $a_i$ reaches a state where $q \in \condemned$ and so, a transition corresponding
  to a matched send to $q$ can not exist from this state and after. Then, $a_j$ is
  not a matched send.
\end{itemize}
Therefore, $\func{w}{\varepsilon}$ is a linearization of
$MSC(\func{w}{\varepsilon})$ validating conditions of causal delivery and so
$MSC(\func{w}{\varepsilon})$ verifies causal delivery.



  Let $\system$ be a system, $\triple$ be a triple of global states of $\system$ and $w \in \LangSRauto$.
  By contradiction, suppose that
  $msc(\func{w}{\varepsilon})$ does not verify causal delivery.  Then, by
  definition of causal delivery, $\func{w}{\varepsilon}$, as all linearizations
  of $msc(\func{w}{\varepsilon})$, contains events $i \prec j$ such that:
  \begin{itemize}
    \item $a_i = \send{p}{q}{\amessage}$ and $a_j = \send{p'}{q}{\amessage'}$;
    \item $a_j$ is matched;
    \item either $a_i$ is unmatched, or there is $i',j'$ such that $a_i \matches a_{i'}$, $a_j \matches a_{j'}$ and $j' \prec i'$.
  \end{itemize}
  So,
  \begin{itemize}
    \item either $a_i$ is unmatched, then as $i \prec j$,
    $w = w_1 \cdot
    \Action{!}{\Message{\amessage}{p}{q}} \cdots
    \Action{!?}{\Message{\amessage'}{p'}{q}} \cdot w_2$. However, after the
    transition labelled $\Action{!}{\Message{\amessage}{p}{q}}$, all reachable states of $\AutSRauto$ have $q \in \condemned$. Then, the
    transition labelled $\Action{!?}{\Message{\amessage'}{p'}{q}}$ cannot happen
    after.  So $w \notin \LangSRauto$ which is a contradiction.
    \item or $j'\prec i'$, but the send and the reception of the same message cannot be separated in $\AutSRauto$.
    Function $f$ put receptions according to send order, and so we cannot have $\func{w}{\varepsilon} = e_1 \cdot \send{p}{q}{\amessage} \cdots \send{p'}{q}{\amessage'} \cdots $ $\rec{p'}{q}{\amessage} \cdots \rec{p}{q}{\amessage'}$ which concludes this proof. \qed
  \end{itemize}

\end{proof}


==> proof_lemma_rcd_cycleSS.tex <==
\begin{quote}
  {\bf Lemma 4}

  For $r \in \decompsetauto$ and for some $\Br$, $ \ecgraph{r,\Br}$ does not
  contains SS cycle iff  for some $\Br'$ $(\globalstateli,\Br)
  \transitionKER{r}{\globalstatelj} (\globalstatelf,\Br')$.

\end{quote}

\begin{proof}

$\Rightarrow$

Suppose that $\ecgraph{r,\Br}$ does not contain an SS cycle. By
contradiction, suppose that
there is no $(\globalstatelf,\Br')$ such that $(\globalstateli,\Br)
\transitionKER{r}{\globalstatelj} (\globalstatelf,\Br')$ and so
there exists $p \in \procSet$ such that $p \in \Crxp{R}{p}'$.
Process $p$ can be added to $\Crxp{R}{p}'$ for different reasons:
\begin{itemize}
\item $p \in \Crxp{R}{p}$ and then there is $\lambdanode_p \cgedgeD{SS}
\lambdanode_p$, by construction of summary nodes edges;
\item $p \in \Crxp{R}{q}$, $v \cgedgeD{SS} \lambdanode_q$ and $
\procofaction{R}{v} = p$, then, independently of whether $v$ is matched or not,
we have $ \lambdanode_q \cgedgeD{SS} v$, by construction of summary nodes edges;
\item $p \in \Crxp{R}{q}$ and $\lambdanode_p \cgedgeD{SS} \lambdanode_q$ and so
we have $\lambdanode_q \cgedgeD{SS} \lambdanode_p$ by construction of summary
nodes edges;
\item there is $v'$ such that $\procofaction{R}{v'} = p $ and $\lambdanode_p
\cgedgeD{SS} v'$ and so there is $v' \cgedgeD{SS} \lambdanode_p$ by construction
of summary nodes edges.
\end{itemize}
Therefore, if $p \in \Crxp{R}{p}'$ then in all cases there is an SS cycle which leads to a
contradiction and concludes this part of the proof.

$\Leftarrow$

Suppose that there is $\Br'$ such that $(\globalstateli,\Br)
\transitionKER{r}{\globalstatelj} (\globalstatelf,\Br')$. By
contradiction, suppose that there is an SS cycle in $\ecgraph{r,\Br}$.  This
means that there is an unmatched message to process $p$, either in $r$, or in
the past, which is causally followed by a matched message $v'$ sent to $p$.
\begin{itemize}
\item Either $v,v'$ appear in $r$ and so we have $v \cgedgeD{SS} v'$ with $v \in
\mathsf{Unm}_p$ and $v$ matched so $\procofaction{R}{v'}= p \in \Crxp{R}{p}'$;
\item or $v$ does not appear in $r$ and so we have $\lambdanode_p \cgedgeD{SS}
v' \cgedgeD{SS} \lambdanode_p$. As $\lambdanode_p \in \mathsf{Unm}_p$ and $v$ is
matched, $p \in \Crxp{R}{p}'$;
\item or neither of them belongs to $r$ and so $p \in \Crxp{R}{p}$ and so $p \in
\Crxp{R}{p}'$.
\end{itemize}
 Therefore, if there is an SS cycle, there exists $p \in \Crxp{R}{p}'$ and so
there is no $\Br'$ such that $(\globalstateli,\Br)
\transitionKER{r}{\globalstatelj} (\globalstatelf,\Br')$ which is a
contradiction and concludes the proof. \qed
\end{proof}


==> proof_theorem_algo.tex <==
\begin{quote}
  {\bf Theorem 5}
  A given system $\system$ is \kSable{k} iff $synchronizable(\system) = k'$
  and $kSynchronizable(\system,k') = True$ with $k' < \infty$.
\end{quote}

\begin{proof}
$\Leftarrow$
Follows from \cite{DBLP:conf/fossacs/GiustoLL20}.

$\Rightarrow$
Let $\system$ be a \kSable{k} system.
As $\system$ is \kSable{k}, for all execution $e \in asEx(\system)$,
$\cgraph{e}$ has SCC of size at most $k$. Assume that $k$ is the smallest.
By contradiction, suppose that the implication is wrong and so:
\begin{itemize}
   \item either $synchronizable(\system) = k' = -1$. In this case,
   there is a triple $\triple$ such that $ \exists r \in \decompreachsetauto$
   and $\cgedgeS \in SCC \in \cgraph{r}$.
   By Theorem~\ref{theorem:large_not_ksynchro}, $\system$ is not \kSable{k} for
   any $k$, which is a contradiction.
%      Let $r \proj{SCC}$ the regular
%    expression $r$ with only messages that belong to the SCC.
%    Since $r$ and $r \proj{SCC}$ are regular and $\cgedge{\star} \in SCC$,
%    we know that, by the Pumping Lemma,
%   there is $N$ such that for all $w \in \Language{r\proj{SCC}}$ of length greater than $N$,
%   there is $x,y,z$ with $w = xyz$ such that $y$ is non empty and of length lower than $N$
%   and $ xy^nz \in \Language{r\proj{SCC}}$ with $n \geq 0$.
%    If $w' = xy^nz$ with $n>k$ then there is $w''$ an extension of $w'$ such that
%    $w'' \in \Language{r}$.
% %   $w'' \in \Language{r}$ such that $w'$ is the projection of $w''$.
%    But $\cgraph{w''}$ has an SCC of size $n >k$ and so we have a
%    contradiction.


  \item or $synchronizable(\system) = k' $ and $kSynchronizable(\system, k') = False$. In
  thise case, there is an execution $e \in asEx(\system)$ such that $e$ is a
  borderline violation:
  \begin{itemize}
    \item either $\cgraph{e}$ contains an SCC with a size greater than $k'$.
    \begin{itemize}
      \item If $k'\geq k$, there is a contradiction because all executions have
      SCC of maximal size $k$.
      \item Otherwise, then $k' < k$.
      Take $e = e_1 \cdots e_n$ an \kSable{k} execution such that
      there exists $e_i$ a \kE{k} with $\size{e_i}= k$.
      As $e$ is a sequence of
      exchanges, we have $(\globalstate{l_0}, B_{\emptyset})
      \transitionKE{e_1}{k} \cdots (\globalstateli, B)\transitionKE{e_i}{k}
      (\globalstatelj,B')$. By Theorem~\ref{theorem:cd_rcd}, there is
      $\globalstatelj$, $\Br'$, $r\in \decompsetauto$ and $w \in
      \Language{r}$ such that $MSC(e_i) = MSC(\func{w}{\varepsilon})$ and
      $(\globalstateli,B) \transitionKER{r}{\globalstatelj}
      (\globalstatelf,\Br')$. As $\triple$ is reachable with $B$, $r \in
      \decompreachsetauto$. $\size{e_i} = k $, then the size of the biggest
      SCC in $\cgraph{\func{w}{\varepsilon}}$ is $k$ and $\size{w} = k$.

      We want to establish a lower bound for $\size{r}$.
      Suppose by contradiction that $\size{r} = k'' < k$.
      Then, by Theorem~\ref{theorem:k_bound},
      $\size{w} \leq k'' < k$ which is a contradiction.

      Therefore, $\size{r} \geq k$.
      Finaly, as $synchronizable(\system)= k'$ with
      $k' < k$, then the $k'$ is the maximal size of a triple in the system,
      which is a contradiction.
    \end{itemize}

    \item or $\cgraph{e}$ contains an SCC with a label RS. Then, $e$ can not be
    devided into \kE{k}, and $\system$ is not \kSable{k} for any $k$ which is a
    contradiction.
  \end{itemize}


\end{itemize}


%
%   Let $\system$ be a system. We can compute $k = max \{ (\size{\triple}) \mid
%   \triple \mbox{ is a reachable triple } \}$. Thanks to
%   Theorem~\ref{theorem:cd_rcd} and Theorem~\ref{theorem:rcd_cd}, we can ensure
%   that all observed triple, and so reachable triple, is runnable by the system
%   and that all triple runnable by the system is a reachable triple and so is
%   observed.
%     If $k \neq \infty$, then for each
%   triple, the biggest possible exchange is of size at most $k$, and for each
%   triple, we know by Lemma~\ref{lemma:k_max} that there is no exchange with a
%   size greater than $k$. So, if the system is not \kSable{k}, there is no no $k'
%   > k$ such that $\system$ \kSable{k'}. As \kSity{k} is decidable for a given
%   $k$, we can test and know whether $\system$ is \kSable{k}.
%   Else, we have $ k = \infty$, so there is an abritrary large reachable triple,
% and by definition, an arbitrarily large "exchange" and, by
% Theorem~\ref{theorem:large_not_ksynchro}, $\system$ is not \kSable{k} for any
% $k$.
\end{proof}


==> proof_theorem_cd_rcd.tex <==
\begin{quote}
  {\bf Theorem 1}
  For a system $\system$, for all $\globalstateli, \globalstatelf, B,
  B'$, for all sequence of actions $e$ and
  $k \in \mathbb{N}$, if
  $(\globalstateli,B) \transitionKE{e}{k} (\globalstatelf, B')$ then there is
  $\globalstatelj, \Br', r \in \decompsetauto$ and $w \in \Language{r}$
  such that $\MSC(e) = \MSC(\func{w}{\varepsilon})$ and $(\globalstateli, B)
  \transitionKER{r}{\globalstatelj} (\globalstatelf,\Br')$.
\end{quote}



\begin{proof}
Let $e$ be a sequence of actions such that $(\globalstateli,B)
\transitionKE{e}{k} (\globalstatelf,B')$. By definition of
$\transitionKE{e}{k}$, $e = s_1 \cdots s_n \cdot r_1 \cdots r_n'$ with $s_1
\cdots s_n \in S^*$, $r_1 \cdots r_n' \in R^*$, and so we can set
$\globalstatelj$ such that
$(\globalstateli,\B_{\emptyset}) \xRightarrow{s_1 \cdots s_n}
(\globalstatelj, \B) \xRightarrow{r_1 \cdots r_n'} (\globalstatelf,\B')$
for some  $\B,\B'$.
By Lemma~\ref{lemma:Aut_SR}, there is a $w \in \LangSRauto$ such that
$\MSC(e) = \MSC( \func{w}{\varepsilon})$ and, by Lemma~\ref{lemma:SR_D}, there
exist at least one $r \in \decompsetauto$ such that $w \in \Language{r}$.

By contradiction, assume that for all $r_k \in \decompsetauto$ such that $w
\in \Language{r_k}$, transition $\transitionKER{r_k}{\globalstatelj}$ is
not valid and so $\exists p \in \procSet$ such that $ p \in \Crxp{R}{p}'$.
If there is $p \in \Crxp{R}{p}'$ then there is a cycle SS in $\ecgraph{r_k,\Br}$
by Lemma~\ref{lemma:rcd_cycleSS}. Let $r_0$ be the smallest decomposition in
$\decompsetauto$ (where the number of vertices in the conflict graph is the
smallest) such that $w \in \Language{r_0}$.
Let $v_1 \cdots v_n$ be the smallest SS cycle in $\ecgraph{r_0,\Br}$ such that $v_1
\cgedgeD{SS} v_n \cgedgeD{SS} v_1$. As $r_0$ is the smallest regular expression,
each vertex that belongs to $\ecgraph{r_0,\Br}$ belongs to
$\cgraph{\func{w}{\varepsilon},B)}$ (the extended conflict graph of the sequence
of actions $\func{w}{\varepsilon}$) too.
Now, there are two posibilities:
\begin{itemize}
\item either $\exists 1\leq i \leq n, q \in \procSet$ such that $v_i =
\lambdanode_q$, and, w.l.o.g, suppose that $v_1 = \lambdanode_q$.
$v_n \cgedgeD{SS} \lambdanode_q$ implies that:
\begin{itemize}
\item Either $v_n$ is matched and $\receiver{v_n} = q$. In this case,
$\lambdanode_q \cgedgeD{SS} v_n$ implies that:
\begin{itemize}
\item either $\sender{v_n} \in \Crxp{S}{q}$, there is $v'$ unmatched such that
$v' \cgedgeD{SS} v_n$ and $\receiver{v'}=q$. So
$\send{\amessage'}{\sender{v'}}{q} \prec
\send{\amessage_n}{\sender{v_n}}{q}$.
But, as $v'$ is unmatched, $v$ matched and $\receiver{v'} = \receiver{v_n}$, we
have also that $\send{\amessage_n}{\sender{v_n}}{q} \prec
\send{\amessage'}{\sender{v'}}{q} $. As $v_n$ and $v'$ are also in $w$, then
this prevent us to have  $(\globalstateli,B)
\transitionKE{f(w,\varepsilon)}{k} (\globalstatelf,B')$ for any $k, B'$ and
this is a contradiction;

\item or $\sender{v_n} \in \Crxp{R}{q}$ then there is $v',v''$ such that $v'
\cgedgeD{SS} v''$, $v'$ unmatched and $\receiver{v'} = q$ and $ \receiver{v''} =
\sender{v_n}$, and we have $\send{\amessage'}{\sender{v'}}{q} \prec
\send{\amessage''}{\sender{v''}}{\receiver{v''}} $ and $
\rec{\amessage''}{\sender{v''}}{\receiver{v''}} \prec
\send{\amessage_n}{\sender{v_n}}{q}$.
As previously, as $v'$ is unmatched and $v_n$ is matched, this leads to a
contradiction;

\item or $\receiver{v_n} \in \Crxp{R}{q}$ then there is $v'$ unmatched such that
$v' \cgedgeD{SS} v$, $\receiver{v'} = q$ and $v$ is matched. And so,
$\send{\amessage'}{\sender{v'}}{q} \prec \send{\amessage_n}{\sender{v_n}}{q}$.
But, as previously,  $\send{\amessage_n}{\sender{v_n}}{q} \prec
\send{\amessage'}{\sender{v'}}{q} $ which leads to a contradiction.
\end{itemize}

\item or $\exists s \in \procSet $ such that $v_n = \lambdanode_s$ . As $v_1 =
\lambdanode_q$ then $q \in C'_{R,q}$ and so we cannot have
$(\globalstateli,B) \transitionKE{f(w,\varepsilon)}{k}
(\globalstatelf,B')$.
\end{itemize}

\item or $ \forall i$, $v_i \neq \lambdanode_q$:
\begin{itemize}
\item either $v_1,v_n \in w$ then $v_1 \cgedgeD{SS} v_n \cgedgeD{SS} v_1 \in
\cgraph{\func{w}{\varepsilon},B}$ and so $w$ does not verify causal delivery and
we cannot have $(\globalstateli,B) \transitionKE{\func{w}{\varepsilon}}{k}
(\globalstatelf,B')$;
\item  or not all vertices of the cycle SS are part of $w$ then there is a
canonical word $w'$ of $r_0$ such that $v_1, v_n \in w'$. $w'$ has exactly two
unfolding of each star operator.
\begin{itemize}
\item if $w$ contains zero unfolding for at least on star operator, then there
is $r_0'$ smaller than $r_0$, which is a contradiction;
\item  else $w$ contains one unfolding of at least one star operator. Then,
there is in $\cgraph{ \func{w'}{\varepsilon},B}$ $a_0 \cgedgeD{SS} a_1
\cgedgeD{SS} b$ such that $a_1$ does not belongs to $w$ and $a_0, a_1, b$ belong
to the SS cycle $v_1 \cdots v_n$. Then $\send{a_0}{q}{r} \prec \send{a_1}{q}{r}$
and $\send{a_1}{q}{r} \prec \send{b}{q'}{r'}$. $a_0$ has the same sender and
receiver as $a_0$. Delete $a_1$ does not change the order on $\send{a_0}{q}{r}
\prec \send{b}{q'}{r'}$ as it does not due to $a_1$, and so there is $a_0
\cgedgeD{SS} b$   in $\cgraph{\func{w}{\varepsilon},B}$.
All edges in the SS cycle are so present in $\cgraph{\func{w}{\varepsilon},B}$
and $w$ does not verify causal delivery and cannot valid  $(\globalstateli,B)
\transitionKE{\func{w}{\varepsilon}}{k} (\globalstatelf,B')$ for any $k,B'$,
which concludes this proof.
\end{itemize}
\end{itemize}
\end{itemize}

As each case leads to a contradiction, then we can conclude that we have
$(\globalstateli,\Br) \transitionKER{r}{\globalstatelj} (\globalstatelf,
\Br')$ for some $\Br, \Br'$. \qed
\end{proof}


==> proof_theorem_k_bound.tex <==
\begin{quote}
  {\bf Theorem 3}
    For $r$ a regular expression without choice operator, $\size{r} = k \neq \infty$
  if and only if for all $w \in \Language{r}$, all SCC in
  $\cgraph{\func{w}{\varepsilon}}$ are of size at most $k$.
\end{quote}

\begin{proof}
$\Rightarrow $

Let $r$ be a regular expression without choice operator such that $\size{r} = k
\neq \infty$. Then, by Def.~\ref{def:size_triple}, $\scgraph{r}$ does not
contain SCC of size greater than $k$.
By contradiction, suppose that there is $w \in \Language{r}$ such that
$\cgraph{\func{w}{\varepsilon}}$ contains an SCC of size $k' >k$.
$\cgraph{\func{w}{\varepsilon}}$ has a bigger SCC than $\scgraph{r}$ so
$w$ is bigger than the canonical word of $r$.
So there is more messages which can be added only by repetition because of a
star in the SCC.
Then, there is a star edge in the SCC of $\scgraph{r}$ such that concerned
messages are repeated most as two times in $w$.
Therefore, the SCC in $\scgraph{r}$ contains a star edge and so $\size{r} =
\infty$ which is a contradiction.

$\Leftarrow$

Let $r$ a regular expression without choice operator such that $\forall w \in
\Language{r}$, $\cgraph{\func{w}{\varepsilon}}$ has no SCC of size greater than
$k$. By contradiction, suppose that $\size{r} = \infty$. Then, there is a star
edge in an SCC of $\scgraph{r}$. So, there exists a $w \in \Language{r}$ such
that a message concerned by a star is repeated $k+1$ times, then
$\cgraph{\func{w}{\varepsilon}}$ contains an SCC of size $k' \geq k+1 >k$ which
is a contradiction and concludes this proof. \qed
\end{proof}


==> proof_theorem_large_not_ksynchro.tex <==
\begin{quote}
  {\bf Theorem 4}

  For a given system $\system$, if there is a reachable triple $\triple$ such that
  there exists $r \in \decompreachsetauto$  such that $\size{r} = \infty$
  then $\system$ is not \kSable{k} for any $k$.

\end{quote}

\begin{proof}
Let $\system$ be a system and $\triple$ be a triple such that $\exists r \in
\decompreachsetauto$ with $\size{r} = \infty$.
  By contradiction, suppose that $\system$ is \kSable{k}.
Since $r \in \decompreachsetauto$, there is $\Br, \Br'$ such that
  $(\globalstateli, \Br) \transitionKER{r}{\globalstatelj} (\globalstatelf, \Br')$
  and $\globalstateli$ is reachable with $\Br$.
As $\size{r} = \infty$, there is an SCC in $\cgraph{r}$ that contains an edge $\cgedgeS$.
Let $r \proj{SCC}$ be the regular expression $r$
with only messages that belong to the SCC. Since $r$ and $r \proj{SCC}$ are
regular and $\cgedgeS \in SCC$, we know that, by the Pumping Lemma,
there is $N$ such that for all $w \in \Language{r\proj{SCC}}$ of length
greater than $N$, there is $x,y,z$ with $w = xyz$ such that $y$ is non empty
and of length smaller than $N$ and $ xy^nz \in \Language{r\proj{SCC}}$ with $n
\geq 0$. Take $w' = xy^nz$ with $n>k$ then this word can be completed to obtain a word  $w'' \in \Language{r}$.
  By Theorem~\ref{theorem:rcd_cd}, for all $w \in \Language{r}$,
  there is  $k'$ and $B'$ such that $(\globalstateli,\Br)
  \transitionKE{\func{w}{\varepsilon}}{k'} (\globalstatelf,B')$.
In particular, we have $(\globalstateli,\Br)
\transitionKE{\func{w''}{\varepsilon}}{k'} (\globalstatelf,B')$ for a $B'$ and $k' \geq n >k$.
So $msc(\func{w''}{\varepsilon})$ verifies causal delivery and, as
$\globalstateli$ is reachable with $\Br$, $\func{w''}{\varepsilon}$ is an
exchange of $\system$.
But $\cgraph{w''}$ has an SCC of size $k' >k$, therefore there is an exchange of
size greater than $k$ in $\system$ which is \kSable{k} so we have a
contradiction. \qed
\end{proof}


==> proof_theorem_rcd_cd.tex <==
\begin{quote}
  {\bf Theorem 2}

  For a system $\system$, for all $\globalstateli,\globalstatelj,
  \globalstatelf,\Br,\Br'$, for $r \in \decompsetauto$, if
  $(\globalstateli,\Br) \transitionKER{r}{\globalstatelj}
  (\globalstatelf,\Br')$ then for all $w \in \Language{r}$ there is $k \in
  \mathbb{N}, B'$ such that $(\globalstateli,\Br)
  \transitionKE{\func{w}{\varepsilon}}{k} (\globalstatelf,B')$.

\end{quote}

\begin{proof}


Let $r$ be a  regular expression and $\triple$ a triple such that
$(\globalstateli,\Br) \transitionKER{r}{\globalstatelj}
(\globalstatelf{\Br' })$. We have that $\ecgraph{r,\Br} = (V,E)$.
Let $w \in \Language{r}$,
by Lemma~\ref{lemma:SR_causal}, as $w \in \LangSRauto$ then
$MSC(\func{w}{\varepsilon})$ verifies causal delivery and so
$\cgraph{\func{w}{\varepsilon}}$ does not contains SS cycle (see
\cite{DBLP:conf/fossacs/GiustoLL20}).

By induction on the total number of iterations of star
operators of $w$:
\begin{itemize}
\item  $w$ contains at most two iterations of each star operator.
$\cgraph{\func{w}{\varepsilon},B} = (V',E')$ and we know that $V' \subseteq V$.

If there is $v,v' \in V'$ such that $v \cgedgeD{XY} v' \in E'$, $X,Y \in
\{S,R\}$, as these edges are built from the sender and receiver of the messages
and from order on the actions, so these information are unchanged from $w$ to
$r$ and  then $v \cgedgeD{XY} v' \in E$.

 Assume by contradiction that, $\forall p \in \procSet$, $p \notin
 \Crxp{R}{p}'$, and that $\exists p \in \procSet$ such that $p \in C'_{R,p}$ for
 $w$.

$p$ can be added to $C'_{R,p}$ for different reasons
(Fig~\ref{fig:exchange_transition}):
\begin{itemize}
\item $p \in C_{R,p}$ then $p \in \Crxp{R}{p}$ and we cannot have
$(\globalstateli,\Br) \transitionKER{r}{\globalstatelj}
(\globalstatelf,\Br')$ which is a contradiction;
\item  there is $q \in \procSet$  such that $p \in C_{R,q}$, $\lambdanode_p
\cgedgeD{SS} \lambdanode_q$, so $p \in \Crxp{R}{q}$  as all the others edges is
unchanged, and the edge $\lambdanode_p \cgedgeD{SS} \lambdanode_q$ is also
present in $E$ and $p \in \Crxp{R}{p}'$ , which is a contradiction;
\item there is $q \in \procSet$ and $v \in V'$ such that $p \in C_{R,q}$, $v
\cgedgeD{SS} \lambdanode_q$ and $\receiver{v} = p$, then for the same reason, $p
\in \Crxp{R}{q}$, the edge $v \cgedgeD{SS} \lambdanode_q$ belong to $E$ and,
obviously, $\receiver{v} = p$ and so $ p \in \Crxp{R}{p}'$ which is a
contradiction.
\end{itemize}
Then, for each word $w$ containing at most two iteration of each star operator,
if $p \notin \Crxp{R}{p}'$ then $p \notin C'_{R,p}$ for $w$ and so $w$ verifies
causal delivery and $(\globalstateli,B)
\transitionKE{\func{w}{\varepsilon}}{k} (\globalstatelf,B')$ for some $B, B'$
and $k$.

\item Suppose that $w$ contains $n\geq 2$ iterations for at least one star
operator. Let $w' \in \Language{r}$ such that $w'$ contains $n-1$ iterations for
the same star operator. Suppose that $(\globalstateli,B)
\transitionKE{f(w',\varepsilon)}{k} (\globalstatelf,B')$ for some $k$ and
$B,B'$, $p \notin C'_{R,p}$ and $\cgraph{\func{w'}{\varepsilon},B} = (V,E)$.
We show that adding an iteration for one of star operator does not modify
$C'_{R,p}$ for all $p \in \procSet$.

Assume by contradiction that there is $p \in \procSet$ such that $p \in
C'_{R,p}$ for $w$.

$p$ can be added to $C'_{R,p}$ for different reasons
(Fig~\ref{fig:exchange_transition}):
\begin{itemize}
\item $p \in C_{R,p}$ for $w$ and so also for $w'$, then we can not have
$(\globalstateli,B) \transitionKE{w'}{k} (\globalstatelf,B')$;
\item  there is $q \in \procSet$  such that $p \in C_{R,q}$, $\lambdanode_p
\cgedgeD{SS} \lambdanode_q \in E'$, so $p \in C_{R,q}$ for $w'$ as the edge
$\lambdanode_p \cgedgeD{SS} \lambdanode_q$ is also present in $E$ because
summary nodes are not involved in star iterations  and so $p \in C'_{R,p}$ for
$w'$, which is a contradiction;
\item there is $q \in \procSet$ and $v \in V'$ such that $p \in C_{R,q}$, $v
\cgedgeD{SS} \lambdanode_q$ and $\receiver{v} = p$. If $v \in V$ then the edge
is present in $E$. Else, if $v$ is part of the added iteration, then there is
$v'$ a previous iteration of the same star operator such that $ v' \cgedgeD{SS}
v \cgedgeD{SS} \lambdanode_q \in E'$. As, $v'$ and $v$ have the same sender and
receiver then $v' \cgedgeD{SS} \lambdanode_q \in E$ so $p \in C'_{R,p}$ for $w'$
which is a contradiction.
\end{itemize}
Therefore, if $ p \notin C'_{R,p}$ for $w'$ then $p \notin C'_{R,p}$ for $w$,
which concludes the proof. \qed
\end{itemize}\end{proof}


==> proofs-section-computation-k0.tex <==
\thmcomputationk*
\input{proof-theorem-computation-k}

%% Pas de preuve pour le dernier théorème: si on ne parle pas
%% de complexité, c'est vraiment évident.

%\thmmain*

%\begin{proof}
%    TODO
%\end{proof}


==> proofs-section-rpe.tex <==
\lemmaprimestronglyconnected*
\input{proof-lemma-prime-strongly-connected}


\lemmasciffsinglevertex*
\input{proof-lemma-sc-iff-single-vertex}


\lemfiniteabstraction*
\input{proof-lemma-finite-abstraction}

Before we prove Lemma~\ref{lem:soundness-alpha-automaton}, we need to introduce
a few notions and observations.
Let $G=(V,E,\lambda_S,\lambda_R)$ be a P-graph.
A vertex $v\in V$ is X-covered if for all $p\in\lambda_X(v)$
$p$ is X-redundant. We also say that $v\in V$ is covered if it is
both S-covered and R-covered. A partial abstraction
of $G$ is a graph $G'=(V',E',\lambda_S,\lambda_R)$ such that
\begin{itemize}
\item $V'=\{V_1,\dots,V_n\}$ where each $V_i$ is a (not necessarily maximal)
strongly connected component of $G$, all $V_i$ are disjoints, and
for all $v\in V\setminus\bigcup_{i=1}^nV_i$ $v$ is covered.
\item for all $i,j$, $(V_i,V_j)\in E'$ iff $(v,v')\in E$ for some $v\in V_i$
and some $v'\in V_j$.
\item for all $i,X$, $\lambda_X(V_i)=\bigcup_{v\in V_i}\lambda_X(v)$
\end{itemize}
Intuitively, $G'$ is a partial abstraction of $G$ if it results from a ``partial application'' of the functions $\mergeof{.}$, $\eraseof{.}$, and
$\sweepof{.}$: some vertices of a same SCC are merged, but not necessarily all,
some labels are erased, but not neces\-sarily all, and some vertices are 
sweeped, but not necessarily all. From this observation, it follows
the following: if $G'$ is a partial abstraction of $G$, then $\alpha(G')=\alpha(G)$.

\lemsoundnessalphaautomaton*

\input{proof-lemma-soundness-alpha-automaton}

\thmprimereg*

\input{proof-theorem-prime-reg}



==> sec4.tex <==
% !TEX root = icalp.tex

\subsection*{Construction of $\AutSRauto$  for Example~\ref{example:aut_SR}}

Figure~\ref{figure:automate_SR} below depicts automaton $\AutSRauto$ built in Example~\ref{example:aut_SR}.

\begin{tikzpicture}[>=stealth,node distance=2.5cm,shorten >=1pt,
    every state/.style={text=black, scale =0.6}, semithick, scale= 0.7]
  \begin{scope}[->, yshift = -6cm, node distance=3.8cm, xshift = 6cm]
      \node[rectangle, thick, draw] at (-5.5,4.5) {$\AutSRauto$};
   	\node[state,
    %initial, initial text ={},
    text width=1.2cm, align = center] (q00)
    {$((0,0,0),$ $(2,0,1))$ %$\emptyset$
    };
  	\node[state, right of=q00, text width=1.2cm, align = center] (q10)
    {$((1,0,0),$ $(2,0,1)) $ %$\{r\}$
    };
  	\node[state, right of=q10, text width=1.2cm, align = center] (q20)
    {$((2,0,0),$ $(2,0,1)) $ %$\{r,q\}$
    };
  	\node[state, above of=q20, node distance = 3cm, text width=1.2cm,  align = center] (q30)
    {$((2,0,1),$ $(2,0,1)) $% $  \{r,q\}$
    };
  	\node[state, above of=q10, node distance = 3cm, text width=1.2cm, align = center] (q40)
    {$((1,0,1),$ $(2,0,1)) $ %$ \{r,q\}$
    };
  	\node[state, below of=q10, node distance = 3cm, text width=1.2cm, align = center] (q43)
    {$((1,0,1),$ $(2,1,1)) $ %$\{r\}$
    };
    \node[state, above of=q00, node distance = 3cm, text width=1.2cm, align = center] (q50)
    {$((0,0,1),$ $(2,0,1)) $ %$ \{q\}$
    };
   	\node[state, left of=q00, text width=1.2cm, align = center] (q11)
    {$((1,0,0),$ $(2,0,2)) $ %$\emptyset$
    };
    \node[state, left of=q11, text width=1.2cm, align = center] (q21)
    {$((2,0,0),$ $(2,0,2)) $ %$\{q\}$
    };
  	\node[state, below of=q20, node distance = 3cm, text width=1.2cm, align = center] (q33)
    {$((2,0,1),$ $(2,1,1)) $ %$\{r,q\}$
    };
   	\node[state, above of=q21, node distance = 3cm, text width=1.2cm, align = center] (q31)
    {$((2,0,1),$ $(2,0,2)) $ %$\{q\}$
    };
  	\node[state, right of=q31, text width=1.2cm, align = center] (q41)
    {$((1,0,1), $ $ (2,0,2)) $ %$\{q\}$
    };
  	\node[state, below of=q00, node distance = 3cm, text width=1.2cm, align = center] (q53)
    {$((0,0,1), $ $(2,1,1))$ %$\emptyset$
    };
  	\node[state, below of=q11, node distance = 3cm, text width=1.2cm, align = center] (q42)
    {$((1,0,1), $ $(2,1,2)) $ %$\emptyset$
    };
  	\node[state, below of=q21,node distance = 3cm, text width=1.2cm, align = center, accepting] (q32)
    {$((2,0,1), $ $(2,1,2)) $ %$\{q\}$
    };

   \path (-0.85,-0.85) edge node{} (-0.55,-0.55);

  	\path (q00) edge node[above] {$\Action{!}{\Message{a}{p}{r}}$} (q10);
  	\path (q00) edge node[left] {$\Action{!}{\Message{b}{r}{q}}$} (q50);
  	\path (q00) edge node[above] {$\Action{!?}{\Message{a}{p}{r}}$}  (q11);
  	\path (q00) edge node[left] {$\Action{!?}{\Message{b}{r}{q}}$} (q53);

  	\path (q10) edge node[above] {$\Action{!}{\Message{c}{p}{q}}$} (q20);
  	\path (q10) edge node[left] {$\Action{!?}{\Message{b}{r}{q}}$}  (q43);
   	\path (q10) edge node[left] {$\Action{!}{\Message{b}{r}{q}}$} (q40);

  	\path (q11) edge node[above] {$\Action{!}{\Message{c}{p}{q}}$} (q21);
  	\path (q11) edge  node[left] {$\Action{!}{\Message{b}{r}{q}}$} (q41);
  	\path (q11) edge node [left] {$\Action{!?}{\Message{b}{r}{q}}$} (q42);

  	\path (q20) edge node[left] {$\Action{!}{\Message{b}{r}{q}}$} (q30);

    \path (q21) edge node[left] {$\Action{!}{\Message{b}{r}{q}}$} (q31);

  	\path (q40) edge node[above] {$\Action{!}{\Message{c}{p}{q}}$} (q30) ;

  	 \path (q41) edge node[above] {$\Action{!}{\Message{c}{p}{q}}$} (q31) ;

  	\path (q42) edge node[above] {$\Action{!}{\Message{c}{p}{q}}$} (q32) ;

  	\path (q43) edge node[above] {$\Action{!}{\Message{c}{p}{q}}$} (q33) ;

  	\path (q50)  edge  node[above] {$\Action{!?}{\Message{a}{p}{r}}$} (q41);
  	\path (q50) edge node[above] {$\Action{!}{\Message{a}{p}{r}}$} (q40);

    \path (q53) edge node[above] {$\Action{!}{\Message{a}{p}{r}}$} (q43);
  	\path (q53)  edge node[above] {$\Action{!?}{\Message{a}{p}{r}}$} (q42);

    \path (q21) edge node [left] {$\Action{!?}{\Message{b}{r}{q}}$} (q32);
    \path (q20) edge node [left] {$\Action{!?}{\Message{b}{r}{q}}$} (q33);

  \end{scope}
\end{tikzpicture}
\captionof{figure}{Automaton $\AutSRauto$ of Example~\ref{example:aut_SR}}\label{figure:automate_SR}


\lemmaautSRcorrect*

\input{proof-lemma-SR-correct}

\lemmacausaldel*

\input{proof-lemma-causal-del}
\begin{proposition}\label{proposition:msc_trace_state}
  For all MSC $\msc$, $\msc\in\asTr(\system)$ iff there is
  $\globalstate{l}\in L_{\system}$ and $\Br\in\absBrSetGood$ such that 
  $(\globalstate{l}_0,\Br_{\emptyset})\Tr{\msc}(\globalstate{l},\Br)$.
  \end{proposition}

\begin{proof}
  See~\cite{DBLP:conf/fossacs/GiustoLL20}.
\end{proof}

\thmreachable*
\input{proof-lem-reachable}

